Sum-of-squares lower bounds for planted clique

Finding cliques in random graphs and the closely related "planted" clique variant, where a clique of size k is planted in a random G(n, 1/2) graph, have been the focus of substantial study in algorithm design. Despite much effort, the best known polynomial-time algorithms only solve the problem for k ~ sqrt(n). In this paper we study the complexity of the planted clique problem under algorithms from the Sum-of-squares hierarchy. We prove the first average case lower bound for this model: for almost all graphs in G(n,1/2), r rounds of the SOS hierarchy cannot find a planted k-clique unless k > n^{1/2r} (up to logarithmic factors). Thus, for any constant number of rounds planted cliques of size n^{o(1)} cannot be found by this powerful class of algorithms. This is shown via an integrability gap for the natural formulation of maximum clique problem on random graphs for SOS and Lasserre hierarchies, which in turn follow from degree lower bounds for the Positivestellensatz proof system. We follow the usual recipe for such proofs. First, we introduce a natural "dual certificate" (also known as a "vector-solution" or "pseudo-expectation") for the given system of polynomial equations representing the problem for every fixed input graph. Then we show that the matrix associated with this dual certificate is PSD (positive semi-definite) with high probability over the choice of the input graph.This requires the use of certain tools. One is the theory of association schemes, and in particular the eigenspaces and eigenvalues of the Johnson scheme. Another is a combinatorial method we develop to compute (via traces) norm bounds for certain random matrices whose entries are highly dependent; we hope this method will be useful elsewhere.

==> oldtechnical.tex <==
% !TEX root = main.tex

\section{Bounding norms of local random matrices}\label{sec:localrand}
In this section we shall develop tools for bounding the norms of \emph{locally random} matrices (recall their definition from \sref{sec:outline}) associated with random graphs $G \lfta G(n,1/2)$, proving \cref{clm:maintechnicalL}. The idea behind our bounds is to use the \emph{trace method}. Recall the trace method: for any matrix $R$, for any positive integer $q$, $||R|| \leq \sqrt[2q]{tr(R^{2q})}$ so we can bound $||R||$ by bounding $tr(R^{2q})$. In this section we use the trace method to bound $||R_a||$ in two steps. In \sref{productandconstraint} we develop tools for bounding the trace of high powers of locally random matrices. In \sref{rabounds} we apply these tools to the matrices $\{R_a\}$.%To do so, we shall use the trace method of bounding the trace of large powers of the matrix and shall develop some generic tools for counting various combinatorial quanties which arise frequently in such calculations and might be useful in other scenarios as well.
%--------------------------------------------------------------------------%
\subsection{Product and constraint graphs}\label{productandconstraint}
%--------------------------------------------------------------------------%
In this subsection, we introduce product and constraint graphs, which are a useful way to visualize terms 
for our trace calculations. We use $V$ rather than $I$ for subsets here because we will be viewing the individual elements of each $V$ as vertices.
\begin{definition}
If we are given $V_1, \ldots, V_{q} \subseteq [n]$ and a product $p = \prod_{j}{M_{j}(V_{a_j},V_{b_j})}$ where for all $j$, $a_j,b_j \in [q]$ and 
$M_j \in \mathbb{R}^{{[n] \choose {|V_{a_j}|}} \times {[n] \choose {|V_{b_j}|}}}$, define 
the product multi-graph $P_{\{V_i\},p}$ and the constraint graph $C_{\{V_i\}}$ as follows:
\begin{enumerate}
\item $V(P_{\{V_i\},p}) = \{V_i: i \in [1,q]\}$.
\item $E(P_{\{V_i\},p}) = \{(V_{a_j},V_{b_j}): M_{j}(V_{a_j},V_{b_j}) \text{ is a term in p for some j}\}$. We label each edge $(V_{a_j},V_{b_j})$ with the corresponding $M_j$.
\item $V(C_{\{V_i\}}) = \{(V_i,j): j \in V_i\}$.
\item $E(C_{\{V_i\}}) = \{((V_{i_1},j),(V_{i_2},j)): j \in V_{i_1}, j \in V_{i_2}, V_{i_1} \neq V_{i_2}\}$.
\end{enumerate}
We define the value $v(P_{\{V_i\},p},C_{\{V_i\}})$ of the pair $(P_{\{V_i\},p},C_{\{V_i\}})$ to be 
$v(P_{\{V_i\},p},C_{\{V_i\}}) = p = \prod_{j}{M_{j}(V_{a_j},V_{b_j})}$
\end{definition}
\begin{example}
If $M \in \mathbb{R}^{{[n] \choose {a}} \times {[n] \choose {a}}}$ then $tr(M^{q}) = \sum_{V_1, \cdots, V_{q}}{\prod_{i=1}^{q}{M({V_i},{V_{i+1}})}}$ where 
$V_{q+1} = V_1$. For all $V_1, \cdots, V_q$, letting $p = {\prod_{i=1}^{q}
{M({V_i},{V_{i+1}})}}$, $P_{\{V_i\},p}$ 
is a cycle with vertices $V_1, \cdots, V_q$ whose edges have label 
$M$. $C_{\{V_i\}}$ consists of the elements of $V_1, \cdots, V_q$ 
with edges between whichever elements happen to be equal.
\end{example}
We next prove a generic result bounding the norms of locally random matrices based on the structure of some associated product/constraint graphs; the advantage being that the conditions on the product/constraint graphs will be easier to ascertain in our applications.
\begin{theorem}\label{thm:productgraphtonorm}
Given a matrix $M \in \mathbb{R}^{{[n] \choose {r_1}} \times {[n] \choose r_2}}$, if we can express $tr(({M}M^T)^{q})$ as a sum of terms such that when we look at 
the corresponding product and constraint graphs, the following statements are true 
\begin{enumerate}
\item The number of vertices in each constraint graph is $qx$ for some integer $x \geq 1$.
\item For every product/constraint graph pair with nonzero expected value, the constraint graph has at most 
$qx - qy + z$ connected components for some integers $y$ and $z$ where 
$1 \leq y \leq x$ and $z \geq 0$.
\item For every product/constraint graph pair with nonzero expected value, 
its expected value has magnitude at most $B^{2q}$ for some constant $B$.
\end{enumerate}
then if $n \geq 10$, for all $\epsilon \in (0,1)$, 
$$\pr\left[||M|| > B\cdot \left(ex\Big(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\Big)\right)^y \cdot n^{\frac{x-y}{2}}\right] < \epsilon$$
\end{theorem}
\begin{proof}
We prove this result by obtaining an upper bound on the number of product/constraint graph pairs 
for $tr(({M}M^T)^{q})$ with nonzero expected value. This gives us an upper bound for 
$tr(({M}M^T)^{q})$ which gives us our upper bound on $||M||$.
\begin{definition}
Define $t(n,k,m)$ to be the number of ways to choose a $k$-tuple of elements in $[n]$ so that the number of unique 
elements in the $k$-tuple is at most $m$.
\end{definition}
\begin{lemma}\label{tboundlemma}
If $m \leq k$ then $t(n,k,m) \leq {k \choose {k-m}}{n^{m}}{{m}^{k-m}}$
\end{lemma}
\begin{proof}
We can choose every $k$-tuple $(x_1, \cdots, x_k)$ of elements in $[n]$ which contains at most $m$ distinct elements as follows. 
There must be at least $k-m$ elements which are duplicates of other elements, so we can first choose a set $I$ of $k-m$ indices 
such that for all $i \in I$, $x_i = x_j$ for some $j \notin I$. There are ${k \choose {k-m}}$ choices for $I$. We then choose 
the elements $\{x_j: j \notin I\}$. There are no restrictions on these elements so there are $n^{m}$ choices for these elements. 
Finally, we choose the elements $\{x_i: i \in I\}$. To determine each $x_i$ it is sufficient to specify the $j \notin I$ such that 
$x_i = x_j$. For each $i$ there are $m$ choices for the corresponding $j$, so the number of choices for these elements 
is at most $m^{k-m}$. Putting everything together, the total number of choices is at most ${k \choose {k-m}}{n^{m}}{{m}^{k-m}}$, 
as needed.
\end{proof}
Now note that for all $q$, $E[tr(({M}M^T)^{q})]$ will be the sum of of the expected values of its product/constraint graph pairs. 
For each constraint graph, there are $qx$ vertices, which corresponds to a $qx$-tuple of elements 
in $[n]$. For each product/constraint graph pairs with nonzero expected vlaue, the constraint graph has at most 
$qx - qy + z$ connected components so the corresponding $qx$-tuple can have at most 
$m = qx - qy + z$ distinct elements. If $q > \frac{z}{y}$ then applying \lref{tboundlemma} with 
$k = qx$ and $m = qx - qy + z$, there are at most 
\begin{align*}
{k \choose {k-m}}{n^{m}}{{m}^{k-m}} &\leq {(km)}^{k-m}{n^m} \\
&= (km)^{yq}(km)^{-z}n^{(x-y)q}n^{z} \\
&= (\frac{n}{km})^{z}\left((km)^{y}n^{x-y}\right)^{q} \\
&\leq n^{z}\left((q^2x^2)^{y}n^{x-y}\right)^{q}
\end{align*}
product/constraint graph pairs with nonzero expected value. By our assumptions, each of these product graphs has 
expected value at most $B^{2q}$, so $E[tr(({M}M^T)^{q})] \leq n^{z}\left((q^2x^2)^{y}n^{x-y}\right)^{q}B^{2q}$. 
Thus, for all $q > \frac{z}{y}$, 
$$E[||M||^{2q}] \leq E[tr(({M}M^T)^{q})] \leq n^{z}\left(B(qx)^{y}n^{\frac{x-y}{2}}\right)^{2q}$$
Using Markov's inequality, 
$$\epsilon > P\left(||M||^{2q} > \frac{1}{\epsilon}E[||M||^{2q}]\right) = P\left(||M|| > 
\sqrt[2q]{\frac{1}{\epsilon}E[||M||^{2q}]}\right)$$
Combining these two equations gives
$$P\left(||M|| > \frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}}
(Bx^{y}n^{\frac{x-y}{2}})\right) < \epsilon$$
We will try to minimize $\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}}$ with respect to $q$. 
Setting the derivative to $0$ gives 
$$\left(\frac{y}{q} - \frac{z\ln{n} - \ln{\epsilon}}{2q^2}\right)
\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}} = 0$$
This occurs when $q = \frac{z\ln{n} - \ln{\epsilon}}{2y}$. We need $q$ to be an integer so we set $q$ to be the smallest 
integer which is at least $\frac{z\ln{n} - \ln{\epsilon}}{2y}$. As long as $n \geq 10$ this guarantees that $q > \frac{z}{y}$. 
Now $q < \frac{z\ln{n} - \ln{\epsilon}}{2y} + 1$ and 
$$\left(\frac{n^z}{\epsilon}\right)^{\frac{1}{2q}} \leq 
\left(e^{z\ln{n} - \ln{\epsilon}}\right)^{\frac{y}{z\ln{n} - \ln{\epsilon}}} = e^y$$
Thus, for this $q$, 
$$\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}} \leq e^y\left(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\right)^y$$
Putting everything together, 
$$P\left(||M|| > e^y\left(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\right)^y
(Bx^{y}n^{\frac{x-y}{2}})\right) < \epsilon$$
and rearranging gives the desired result.
\end{proof}
%--------------------------------------------------------------------------%
\subsection{Bounds on $||R_a||$}\label{rabounds}
%--------------------------------------------------------------------------%
We now prove \clref{clm:maintechnicalL} restated here (with more precise constants) for convenience. For this proof, we use \tref{thm:productgraphtonorm}. When we look at the product/constraint graph pairs for $tr(({R_a}{R^T_a})^q)$, every product edge corresponds to a term in the product. Each such term has expected value $0$ by itself and is independent of all other terms unless the constraint edges link it to another term. This will only happen when the product edge is part of what we will call an independence breaking cycle. Now every product/constraint graph pair will have expected value $0$ unless every product edge is part of an independence breaking cycle, so to use \tref{thm:productgraphtonorm} it is sufficient to upper bound the number of connected components in the constraint graph when every product edge is part of an independencce breaking cycle.
\begin{theorem}
If $n \geq 100$, for all $\epsilon \in (0,1)$, 
$\pr\left[||R_a|| > 4a2^{a^2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon$
\end{theorem}
\begin{proof}
Since $R_a$ is symmetric, $tr(({R_a}{R^T_a})^q) = \sum_{V_1, \cdots, V_{2q}}{\prod_{i=1}^{2q}{R_a(V_{i},V_{i+1})}}$ 
where $V_{2q+1} = V_{1}$. Let's consider which product/constraint graph pairs for $tr(({R_a}{R^T_a})^q)$ have expected value $0$.
\begin{definition}
Given $q$ and $\{V_1, \cdots, V_{2q}\}$, we define $V_{i \pm 2q} = V_{i}$ for all $i \in [1,2q]$.
\end{definition}
\begin{definition} For a product constraint graph pair $(P_{\{V_1, \cdots, V_{2q}\},p},C_{\{V_1, \cdots, V_{2q}\}})$ where $q \geq 2$, 
\begin{enumerate}
\item Define an independence breaking 3-cycle to consist of product edges $(V_i,V_{i+1})$, $(V_{i+1},V_{i+2})$ 
and a constraint edge $((V_{i},j),(V_{i+2},j))$.
\item Define an independence breaking 4-cycle to consist of product edges $e_1 = (V_{i_1},V_{i_1+1})$, 
$e_2 = (V_{i_2},V_{i_2 \pm 1})$ and constraint edges $((V_{i_1},j_1),(V_{i_2},j_1))$, 
$((V_{i_1+1},j_2),(V_{i_2 \pm 1},j_2))$. Note that $V_{i_1},V_{i_1+1}$ do not have to be disjoint from 
$V_{i_2},V_{i_2 \pm 1}$
\end{enumerate}
\end{definition}
\begin{proposition}
For all $V_1, \cdots, V_{2q}$, taking $p = \prod_{i=1}^{2q}{R_a(V_{i},V_{i+1})}$ where $V_{2q + 1} = V_1$, 
if $q \geq 2$ and $P_{\{V_i\},p}$ contains a product edge $e$ which is not contained in any independence breaking 
3-cycle or 4-cycle, then $(P_{\{V_i\},p},C_{\{V_i\}})$ has expected value $0$.
\end{proposition}
\begin{proof}
Looking at the product corresponding to the product graph, the term corresponding to $e$ is 
independent of all the other terms and has expected value $0$ so the entire product has expected value $0$, as needed.
\end{proof}
Thus, it is sufficient to bound the number of product/constraint graph pairs such that every product edge $e$ is contained 
in an independence breaking 3-cycle or 4-cycle. We do this with the following lemma.
\begin{lemma}\label{lem:connectedcomponentbound}
If $q \geq 2$ and $(P_{\{V_1, \cdots, V_{2q}\},p},C_{\{V_1, \cdots, V_{2q}\}})$ is a product/constraint graph pair such 
that the product edges form a cycle on $V_1, \cdots, V_{2q}$ and every product edge is contained in an indepepndence breaking 
3-cycle or 4-cycle, then there are at most $|V(C_{\{V_1, \cdots, V_{2q}\}})| - q + 1$ connected components in 
$C_{\{V_1, \cdots, V_{2q}\}}$.
\end{lemma}
The intuitive idea behind this lemma is that if we add the constraint edges in the right order, every new constraint edge can put two product edges into independence breaking cycles. For example, a constraint edge between $V_{i-1}$ and $V_{i+1}$ puts the product edges $(V_{i-1},V_i)$ and $(V_i,V_{i+1})$ into an independence breaking 3-cycle. If we then add a constraint edge between $V_{i-2}$ and $V_{i+2}$, this puts the product edges $(V_{i-2},V_{i-1})$ and $(V_{i+1},V_{i+2})$ into an independence breaking 4-cycle. The final constraint edge can put 4 product edges into independence breaking cycles, so the number of constraint edges needed is $q-1$.

to make this argument work, we use an inductive proof. We note that if there is no $V_i$ whose vertices are all isolated in the constraint graph, we must have at least $q$ constraint edges. On the other hand, if there a $V_i$ whose vertices are isolated, there must be a constraint edge from $V_{i-1}$ and $V_{i+1}$. As noted above, this constraint edge puts the product edges $(V_{i-1},V_i)$ and $(V_i,V_{i+1})$ into an independence breaking 3-cycle. We take this to be the first constraint edge. We then argue that we can essentially delete $V_i$ and merge $V_{i-1}$ and $V_{i+1}$ which allows us to use the inductive hypothesis. We make these ideas rigorous below.
\begin{proof}[Proof of \lref{lem:connectedcomponentbound}]
We prove \lref{lem:connectedcomponentbound} by induction on $q$. The base case $q = 2$ is trivial, as we clearly need at least one constraint edge, so the number 
of connected components in $C_{\{V_1, \cdots, V_{2q}\}}$ is at most the number of vertices in $C_{\{V_1, \cdots, V_{2q}\}}$ minus 1. 
Now assume that $q = k \geq 3$ and the result is true for $q = k-1$. Here we are only looking at the structure of the 
product/constraint graph pair $(P,C)$ so we ignore the product $p$. 

First note that if there is no $V_i$ such that all vertices $(V_i,j)$ in $C_{\{V_1, \cdots, V_{2q}\}}$ are isolated, then there are at most 
$|V(C_{\{V_1, \cdots, V_{2q}\}})| - q$ connected components in $C_{\{V_1, \cdots, V_{2q}\}}$. Thus, we may assume that 
for some $i$, all vertices $(V_i,j)$ in $C_{\{V_1, \cdots, V_{2q}\}}$ are isolated. Now 
note that for the product edge $e = (V_{i-1},V_{i})$, since all vertices $(V_i,j)$ in $C_{\{V_1, \cdots, V_{2q}\}}$ are 
isolated, there are no independence breaking 3-cycles or 4-cycles where $(V_i,j)$ is the endpoint of a constraint edge. 
Thus, we must have that $e$ is part of an independence breaking 3-cycle consisting of $e = (V_{i-1},V_i)$, $e_2 = (V_i,V_{i+1})$, and 
a constraint edge $((V_{i-1},j),(V_{i+1},j))$ for some $j \in V_{i-1} \cap V_{i+1}$.

Now form a new product/constraint graph pair $(P,C)$ as follows. Delete $V_i$ and merge $V_{i-1}$ and $V_{i+1}$ into a new set of 
vertices $W = V_{i-1} \cup V_{i+1}$. More precisely, 
\begin{enumerate}
\item Take $V(P) = V(P_{\{V_1, \cdots, V_{2q}\},p}) \setminus \{V_{i-1},V_i,V_{i+1}\} \cup \{W\}$
\item Take $E(P) = E(P_{\{V_1, \cdots, V_{2q}\},p}) \setminus \{(V_{l},V_{l+1}): l \in [i-2,i+1]\} 
\cup \{(V_{i-2},W),(W,V_{i+2})\}$
\item Take $V(C) = V(C_{\{V_1, \cdots, V_{2q}\}}) \setminus \{(V_{l},j): l \in [i-1,i+1], j \in V_l\} 
\cup \{(W,j): j \in V_{i-1} \cup V_{i+1}\}$
\item Take \begin{align*} E(C) &= E(C_{\{V_1, \cdots, V_{2q}\}}) \setminus 
\{((V_{l_1},j),(V_{l_2},j)): l_1 \in [i-1,i+1], j \in V_{l_1} \cap V_{l_2}\} \\
&\cup \{((W,j),(V_{l_2},j)): l_2 \notin [i-1,i+1], j \in \left(V_{i-1} \cup V_{i+1}\right) \cap V_{l_2}\}
\end{align*}
\end{enumerate}
We now observe that every independence breaking 3-cycle or 4-cycle of $(P_{\{V_1, \cdots, V_{2q}\},p},C_{\{V_1, \cdots, V_{2q}\}})$ 
becomes an independence breaking 3-cycle or 4-cycle of $(P,C)$ except for the ones involving $V_i$. To see this, first note 
that since $q \geq 3$, all independence breaking 3-cycles not involving $V_i$ are unaffected (except that $V_{i-1}$ or 
$V_{i+1}$ might be replaced by $W$). Then note that the only way an independence breaking 4-cycle can become anything other than 
an independence breaking 4-cycle is if the merging of $V_{i - 1}$ and $V_{i + 1}$ contracted a constraint edge. In this case, 
the original 4-cycle must have had $(V_{i-2},V_{i-1})$ and $(V_{i+1},V_{i+2})$ as the two product edges and had constraint edges of the 
form $((V_{i-1},j_1),(V_{i-1},j_1))$, $((V_{i-2},j_2),(V_{i+2},j_2))$. This type of indepence breaking 4-cycle 
in $(P_{\{V_1, \cdots, V_{2q}\},p},C_{\{V_1, \cdots, V_{2q}\}})$ becomes an independence breaking 3-cycle consisting of 
product edges $(V_{i-2},W)$, $(W,V_{i+2})$ and a constraint edge $((V_{i-2},j_2),(V_{i+2},j_2))$, so the claim holds.

This implies that every product edge of $(P,C)$ is contained in an independence breaking 3-cycle or 4-cycle. By the 
inductive hypothesis, $C$ has at most $|V(C)| - q + 2$ connected components. $C$ does not have any of the vertices 
$(V_i,j)$ of $C_{\{V_1, \cdots, V_{2q}\}}$ and we had two distinct vertices $(V_{i-1},j)$ and $(V_{i+1},j)$ of 
$C_{\{V_1, \cdots, V_{2q}\}}$ which became the same vertex $(W,j)$ in $C$, so $|V(C)| \leq 
|V(C_{\{V_1, \cdots, V_{2q}\}})| - |V_i| - 1$. Thus, $C$ has at most $|V(C_{\{V_1, \cdots, V_{2q}\}})| - |V_i| - q + 1$ 
connected components. The number of connected components of 
$C_{\{V_1, \cdots, V_{2q}\}}$ is equal to the number of connected components of $C$ plus $|V_i|$ which is at most 
$|V(C_{\{V_1, \cdots, V_{2q}\}})| - q + 1$, as needed.
\end{proof}
Using \lref{lem:connectedcomponentbound}, we can now apply \tref{thm:productgraphtonorm} with 
$x = 2a$, $y = 1$, and $z = 1$. Every entry of $R_a$ has magnitude at most $2^{a^2}$ so we can take $B = 2^{a^2}$. 
By \tref{thm:productgraphtonorm}, if $n \geq 10$, for every $\epsilon \in (0,1)$, 
$$\pr\left[||R_a|| > 2^{a^2}\left(2ea\Big(\frac{\ln{n} - \ln{\epsilon}}{2} + 1\Big)\right]
n^{\frac{2a-1}{2}}\right) = 
\pr\left[||R_a|| > 2^{a^2}ea(\ln{n} - \ln{\epsilon} + 2)
n^{a - \frac{1}{2}}\right] < \epsilon.$$
Since $4\ln{n} \geq e(\ln{n} + 2)$ for all $n \geq 100$, we have that for all $n \geq 100$,
$$\pr\left[||R_a|| > 4a2^{a^2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon.$$
\end{proof}

%%% Local Variables:   
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> oldtechnical2.tex <==
% !TEX root = main.tex

%--------------------------------------------------------------------------%
\section{Concentration bounds for number of cliques and $deg_G(I)$}\label{sec:degreevariancecalculations}
%--------------------------------------------------------------------------%
In this section, we prove the following large-deviation bounds on the number of $x$-cliques a random $G(n,1/2)$ graph contains and on $deg_G(I)$. While we prove concrete concentration results as we want the precise constants, similar results (which are likely sufficient for our needs) appear in the literature; see \cite{Rucinski88, Vu01, JLR11book} for instance.
\begin{definition}
For a graph $G$, define $N_x(G)$ to be the number of $x$-cliques in $G$.
\end{definition}
\begin{theorem}\label{cliqueboundtheoremone}
For all $\epsilon \in (0,1)$, for all $x$, if $n > {x^2}(2e - e\ln{\epsilon})(2e + 2 - e\ln{\epsilon})$ then 
$$\pr\left[\left|N_x(G) - 2^{-{x \choose 2}}{n \choose x}\right| > 
e(2 - \ln{\epsilon})\frac{x^2}{x!}n^{x-1}\right] < \epsilon.$$
\end{theorem}
\begin{definition}
Given any $I \subseteq [n]$, let $A_I$ be the set of all vertices not in $I$ which are adjacent to all 
vertices in $I$.
\end{definition}
\begin{theorem}\label{cliqueboundtheoremtwo}
For any $I \subseteq [n]$ of size at most $d = 2r$, if $I$ is a clique in $G$ then for any $\epsilon \in (0,1)$, if $n \geq 4{d^2}2^{2d}(3 - \ln{\epsilon})^2$ then
$$\pr\left[\,\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}}\right| > 
8(3 - \ln{\epsilon})n^{d - |I| - \frac{1}{2}}\,\right] < \epsilon$$
More precsiely, if $|I| < d$ then
\begin{align*}
\pr &\left[\,\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - \left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| > \right. \\
&\;\;\;\;\left. 2^{d+4}(3 - \ln{\epsilon})^2n^{d-|I|-1}\,\right] < \epsilon.
\end{align*}
\end{theorem}
\begin{remark}
We do this more precise analysis here because it will be useful in the analysis of the first bound as well.
\end{remark}
The key lemma in proving Theorem \ref{cliqueboundtheoremone} is the following 
lemma which bounds how often cliques of size $x$ share edges.
\begin{lemma}\label{cliqueboundlemma}
If $x \geq 2$ and $n \geq {x^2}q(q+2)$ then there are at most 
$2n^{xq - q}\left(\frac{{x^2}}{x!}\right)^{q}$ multi-sets $S = \{V_1, \cdots, V_q\}$ of $x$-cliques such 
that for all $j$ there exists an $i \neq j$ such that $|V_i \cap V_j| \geq 2$.
\end{lemma}
\begin{proof}
\begin{definition}
For each multi-set $S = \{V_1, \cdots, V_k\}$ of $k$ $x$-cliques, define the constraint graph 
$H_S$ as follows.
\begin{enumerate}
\item $V(H_S) = \{V_1, \cdots, V_k\}$
\item $E(H_S) = \{(V_i,V_j): |V_i \cap V_j| \geq 2\}$
\end{enumerate}
\end{definition}
Let's first bound the number of $S$ such that $H_S$ is connected.
\begin{lemma}\label{connectedcaselemma}
For any $x,k \geq 2$, there are at most 
$n^{kx-2k+2}k!\frac{2}{x^4}\left(\frac{{x^4}}{2(x!)}\right)^{k}$ multi-sets $S$ of $k$ $x$-cliques 
such that $H_S$ is connected.
\end{lemma}
\begin{proof}
Since $H_S$ is connected, we can order $\{V_1, \cdots, V_k\}$ so that for all $j > 1$ there is an $i < j$ such that 
$(V_i,V_j) \in E(H_S)$. Assuming this is the case, we have at most ${n \choose x}$ choices for $V_1$. For each $j > 1$, 
there are two vertices in $V_j$ which are contained in some $i$ where $i < j$. There are at most $j$ choices for this 
$i$ and then there are ${d \choose 2}$ choices for which two vertices of $V_i$ are contained in $V_j$. There are at 
most ${{n} \choose {x-2}}$ choices for the other $x-2$ vertices of $V_j$ so for each $j > 1$ there are at most 
$j{x \choose 2}{{n} \choose {x-2}}$ choices for $V_j$. Putting everything together, there are at most 
$${n \choose x}{k!}\left({x \choose 2}{{n} \choose {x-2}}\right)^{k-1} \leq 
{n^x}\frac{k!}{x!}\left(\frac{{x^4}n^{x-2}}{2(x!)}\right)^{k-1} \leq 
n^{kx-2k+2}k!\frac{2}{x^4}\left(\frac{{x^4}}{2(x!)}\right)^{k}$$
multi-sets $S$ of $k$ $x$-cliques such that $H_S$ is connected.
\end{proof}
Now consider the number of multi-sets $S$ of $q$ $x$-cliques such that $H_S$ has $t$ connected 
components with sizes $s_1, \cdots, s_t$. Using Lemma \ref{connectedcaselemma}, there are at most 
$$\prod_{i=1}^{t}{\left(n^{{s_i}x-2{s_i}+2}{s_i}!\frac{2}{x^4}\left(\frac{{x^4}}{2(x!)}\right)^{{s_i}}\right)} = 
\left(\prod_{i=1}^{t}{{s_i}!}\right){n^{xq - 2q + 2t}\left(\frac{2}{x^4}\right)^{t}\left(\frac{{x^4}}{2(x!)}\right)^{q}}$$
such $S$.

We now total this up over all possible $t,s_1, \cdots, s_t$. For the special case that all connected components 
of $H_S$ have size $2$, there are at most ${n^{xq - q}\left(\frac{{x^2}}{x!}\right)^{q}}$ such $S$. 
We will show that this term contributes more than all of the other terms combined, which implies 
that the total number of $S$ is at most $2{n^{xq - q}\left(\frac{{x^2}}{x!}\right)^{q}}$, as needed.

For a given $t$, $\prod_{i=1}^{t}{{s_i}!} \leq 2^{t-1}{(q+2-2t)!} \leq {2^t}{(q+2)^{q-2t}}$. 
Also, each of the $t$ components of $H_S$ must have at least two vertices so to determine the sizes 
$s_1,\cdots,s_t$ it is sufficient to decide how to distribute the $q-2t$ extra vertices among the $t$ connected 
components of $H_S$. There are at most ${{q - t - 1} \choose {t-1}} \leq q^{q - 2t}$ ways to do this. Thus, the total 
contribution for terms of a given $t$ is at most 
$${2^t}{(q(q+2))^{q-2t}}n^{xq - 2q + 2t}\left(\frac{2}{x^4}\right)^{t}\left(\frac{{x^4}}{2(x!)}\right)^{q} = 
\left(\frac{{x^2}q(q+2)}{2n}\right)^{q - 2t}\left({n^{xq - q}\left(\frac{{x^2}}{(x!)}\right)^{q}}\right)$$

Since $n \geq {x^2}q(q+2)$, the ${n^{xq - q}\left(\frac{{x^2}}{x!}\right)^{q}}$ term which comes from 
$t = \frac{q}{2}$ contributes more than all the other terms combined, as needed.
\end{proof}
Using Lemma \ref{cliqueboundlemma}, we can bound the deviation of the number of $x$-cliques in $G$ from its expected value, proving \tref{cliqueboundtheoremone}.
\begin{definition}
Define $X = \sum_{V: V \subseteq V(G), |V| = x}{\left(1_{V} - 2^{-{x \choose 2}}\right)}$ where $1_V = 1$ if $V$ is a clique in $G$ and 
$0$ otherwise.
\end{definition}
\begin{proposition}
$X = N_x(G) - 2^{-{x \choose 2}}{n \choose x}$
\end{proposition}
\begin{corollary}\label{cliqueboundcorollaryone}
If $x \geq 2$ and $n \geq {x^2}q(q+2)$ then $E[X^q] < 2q!\left(\frac{{x^2}}{x!}n^{x-1}\right)^q$.
\end{corollary}
\begin{proof}
$E[X^q] = \sum_{V_1, \cdots, V_q: \atop \forall i, V_i \subseteq V(G), |V_i| = x}
{E\left[\prod_{i=1}^{q}{\left(1_{V_i} - 2^{-{x \choose 2}}\right)}\right]}$. Note that all terms of this sum have value less than $1$. Furthermore, for all nonzero terms in this sum, 
for all $j$ there must be an $i$ such that $|V_i \cap V_j| \geq 2$. Thus, this sum 
is at most the number of ordered multi-sets of $q$ $x$-cliques $\{V_1, \cdots, V_q\}$ where for all $j$ there 
is an $i$ such that $|V_i \cap V_j| \geq 2$. In turn, this is at most $q!$ times the number 
of unordered multi-sets of such $q$ $x$-cliques. By Lemma \ref{cliqueboundlemma}, this is at most 
$2q!\left(\frac{{x^2}}{x!}n^{x-1}\right)^q$, as needed.
\end{proof}
We are now ready to prove Theorem \ref{cliqueboundtheoremone}.
\ignore{ which we restate here for convenience.
\vskip.1in
\noindent
{\bf Theorem \ref{cliqueboundtheoremone}.}
{\it
For all $\epsilon \in (0,1)$, for all $x$, if $n > {x^2}(2e - e\ln{\epsilon})(2e + 2 - e\ln{\epsilon})$ then 
$$P\left[\left|N_x(G) - 2^{-{x \choose 2}}{n \choose x}\right| > 
e(2 - \ln{\epsilon})\frac{x^2}{x!}n^{x-1}\right] < \epsilon$$
}}
\begin{proof}[Proof of \tref{cliqueboundtheoremone}]
The result is trivial for $x = 0$ and $x = 1$ so we may assume that $x \geq 2$. 
Using Corollary \ref{cliqueboundcorollaryone} and Markov's inequality, 
$$\epsilon > P\left[X^q > \frac{E[X^q]}{\epsilon}\right] \geq 
P\left[X^q > \frac{2q!\left(\frac{{x^2}}{x!}n^{x-1}\right)^q}{\epsilon}\right] 
= P\left[|X| > \sqrt[q]{\frac{2q!}{\epsilon}}\frac{x^2}{x!}n^{x-1}\right]$$

Thus, we just need to give an upper bound on $\min_{\{\text{positive even q}\}}\{\sqrt[q]{\frac{2q!}{\epsilon}}\}$. 
For all positive even $q$, $2q! \leq q^q$ so this expression is upper bounded by $\frac{q}{\sqrt[q]{\epsilon}}$. 
We now try to minimize $\frac{q}{\sqrt[q]{\epsilon}}$ over all positive even $q$. Taking the derivative of this expression 
with respect to $q$ yields $\frac{1}{\sqrt[q]{\epsilon}} + \frac{\ln{\epsilon}}{q\sqrt[q]{\epsilon}}$. Setting this 
to $0$ yields $q = -\ln{\epsilon}$. However, we require $q$ to be even so we take $q$ to be the smallest positive even 
integer which is greater than $-\ln{\epsilon}$. Now $q < 2 - \ln{\epsilon}$ and 
$\sqrt[q]{\epsilon} \geq \sqrt[(-\ln{\epsilon})]{\epsilon} = \left(e^{\ln{\epsilon}}\right)^{\frac{1}{-\ln{\epsilon}}} = \frac{1}{e}$. 
Putting everything together, for this $q$, $\sqrt[q]{\frac{2q!}{\epsilon}} \leq \frac{q}{\sqrt[q]{\epsilon}} < 2e - e\ln{\epsilon}$. 
Plugging this in gives 
$$\epsilon > P\left[|X| > \sqrt[q]{\frac{2q!}{\epsilon}}\frac{x^2}{x!}n^{x-1}\right] \geq 
P\left[|X| > e(2-\ln{\epsilon})\frac{x^2}{x!}n^{x-1}\right]$$
All that is left is to check that $n \geq {x^2}q(q+2)$ for this $q$ to make sure that our application of 
Corollary \ref{cliqueboundcorollaryone} was valid. Since $n > {x^2}(2e - e\ln{\epsilon})(2e + 2 - e\ln{\epsilon})$, this holds, 
as needed.
\end{proof}
Now that we have proven Theorem \ref{cliqueboundtheoremone}, we will derive Theorem \ref{cliqueboundtheoremtwo} 
from Theorem \ref{cliqueboundtheoremone}. The idea is that conditioned on $I$ being a clique, by 
Theorem \ref{cliqueboundtheoremone}, $deg_G(I)$ is primarily determined by $|A_I|$, which can be easily shown to be tightly concentrated around its expected value. %and this is expected to deviate by a factor of $\Theta(\sqrt{n})$ from its expected value. 
We make this argument rigorous below.
\ignore{
\vskip.1in
\noindent
{\bf Theorem \ref{cliqueboundtheoremtwo}.}
{\it
For any $I \subseteq [n]$ of size at most $d = 2r$, if $I$ is a clique in $G$ then for any $\epsilon \in (0,1)$, if $n \geq 4{d^2}2^{2d}(3 - \ln{\epsilon})^2$ then
$$P\Big(\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}}\right| > 
8(3 - \ln{\epsilon})n^{d - |I| - \frac{1}{2}}\Big) < \epsilon$$
More precsiely, if $|I| < d$ then
\begin{align*}
P\Big(&\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| > \\
&2^{d+4}(3 - \ln{\epsilon})^2n^{d-|I|-1}\Big) < \epsilon
\end{align*}
}}
\begin{proof}[Proof of \tref{cliqueboundtheoremtwo}]
The result is trivial if $|I| = d$ and follows immediately from Theorem \ref{cliqueboundtheoremone} if $|I| = 0$ 
so we may assume that $0 < |I| < d$. Before proving the probabilistic bounds on $deg_G(I)$, we first 
prove probabilistic bonds on $deg_G(I)$ for a given $|A_I|$.
\begin{lemma}\label{ndvavassumedlemma}
If $n > d$ then for any $I \subseteq [n]$ of size less than $d$, if we first determine all of the edges 
incident to elements of $I$ (which determines $A_I$) then if $I$ is a clique, when we look at the remainder of the graph, for any $\epsilon_1 \in (0,1)$, 
\begin{align*}
P\Big(&\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| > \\
&10(2 - \ln{\epsilon_1})n^{d-|I|-1} + (d - |I|)^2\left(\frac{2^{|I|}|A_I|}{n-|I|} - 1\right)^2
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!}\Big) < \epsilon_1
\end{align*} 
so long as the following conditions hold:
\begin{enumerate}
\item $(d - |I|)\left|\frac{2^{|I|}|A_I|}{n - |I|} - 1\right| \leq 1$
\item $|A_I| > {d^2}(2e - e\ln{\epsilon_1})(2e + 2 - e\ln{\epsilon_1})$
\end{enumerate}
\end{lemma}
\begin{proof}
We break $$deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}$$ 
into four parts and analyze each one separately.
\begin{enumerate}
\item $2^{{{|I|} \choose 2} - {d \choose 2}}\frac{(n - |I|)^{d - |I|}}{(d-|I|)!} - 2^{{{|I|} \choose 2} - 
{d \choose 2}}{{n-|I|} \choose {d - |I|}}$
\item $2^{-{{d - |I|} \choose 2}}\frac{|A_I|^{d - |I|}}{(d - |I|)!} - 
2^{{{|I|} \choose 2} - {d \choose 2}}\frac{(n - |I|)^{d-|I|}}{(d - |I|)!} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n - |I|)^{d-|I|-1}}{(d-|I|-1)!}$
\item $2^{-{{d - |I|} \choose 2}}{{|A_I|} \choose {d-|I|}} - 2^{-{{d - |I|} \choose 2}}\frac{|A_I|^{d - |I|}}{(d - |I|)!}$
\item $deg_G(I) - 2^{-{{d - |I|} \choose 2}}{{|A_I|} \choose {d-|I|}}$
\end{enumerate}
\begin{lemma}\label{ndvpartonelemma}
If $n > d \geq |I|$ then $\left|2^{{{|I|} \choose 2} - {d \choose 2}}\frac{(n - |I|)^{d - |I|}}{(d-|I|)!} - 
2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}}\right| \leq 2^{{{|I|} \choose 2} - {d \choose 2}}n^{d - |I| - 1}$
\end{lemma}
\begin{proof}
\begin{proposition}\label{factorialapproxprop}
For all nonnegative integers $n$ and $k$ where $k < n$, $0 \leq \frac{n^k}{k!} - {n \choose k} \leq \frac{k^2}{2n}\frac{n^k}{k!}$
\end{proposition}
\begin{proof}
Note that $n^k \geq \prod_{j=0}^{k-1}{(n-j)} \geq n^k\prod_{j=0}^{k-1}{(1 - \frac{j}{n})} \geq 
n^k(1 - \sum_{j=0}^{k-1}{\frac{j}{n}}) \geq n^k(1 - \frac{k^2}{2n})$

This implies that $0 \leq n^k - \prod_{j=0}^{k-1}{(n-j)} \leq \frac{k^2}{2n}{n^k}$ and dividing everything by 
$k!$ gives the claimed result.
\end{proof}
Applying Proposition \ref{factorialapproxprop} on $n - |I|$ and $d - |I|$ gives 
$$\left|\frac{(n-|I|)^{d - |I|}}{(d - |I|)!} - {{n - |I|} \choose {d - |I|}}\right| \leq 
\frac{(d - |I|)^2}{2(n - |I|)}\frac{(n - |I|)^{d - |I|}}{(d - |I|)!} \leq (n - |I|)^{d - |I| - 1} \leq n^{d - |I| - 1}$$
Multiplying this equation by $2^{{{|I|} \choose 2} - {d \choose 2}}$ gives the claimed result.
\end{proof}
\begin{lemma}\label{ndvparttwolemma}
If $(d - |I|)\left|\frac{2^{|I|}|A_I|}{n - |I|} - 1\right| \leq 1$ then
\begin{align*}&\left|2^{-{{d - |I|} \choose 2}}\frac{|A_I|^{d - |I|}}{(d - |I|)!} - 
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| \\
&\leq (d - |I|)^2\left(\frac{2^{|I|}|A_I|}{n-|I|} - 1\right)^2
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!}\end{align*}
\end{lemma}
\begin{proof}
\begin{proposition}\label{exponentprop}
For all nonnegative integers $x$ and $d$ where $x \leq d$, $x(d-x) + {x \choose 2} - {d \choose 2} = -{{d-x} \choose 2}$. 
\end{proposition}
\begin{proof}
Rearranging this equation gives ${d \choose 2} = {x \choose 2} + dx + {{d-x} \choose 2}$ which just says that 
if we want to pick two elements in $[1,d]$ we can either pick two elements in $[1,x]$, one element from $[1,x]$ and 
one element from $[x+1,d]$, or two elements from $[x+1,d]$. 
\end{proof}
\begin{proposition}
For any nonnegative integer $k$ and any $x$ such that $|kx| \leq 1$, $\left|(1+x)^k - (1 + kx)\right| \leq {k^2}{x^2}$
\end{proposition}
\begin{proof}
$$\left|(1+x)^k - (1 + kx)\right| \leq \sum_{j=2}^{k}{\left|{k \choose j}{x^j}\right|} 
\leq \sum_{j=2}^{k}{\left|\frac{1}{j!}{k^j}{x^j}\right|} \leq {k^2}{x^2}\sum_{j=2}^{k}{\frac{1}{j!}} \leq {k^2}{x^2}$$
\end{proof}
Applying this proposition with $x = \frac{2^{|I|}|A_I|}{n-|I|} - 1$ and $k = (d - |I|)$, since 
$(d - |I|)\left|\frac{2^{|I|}|A_I|}{n - |I|} - 1\right| \leq 1$, 
$$\left|\frac{2^{|I|(d - |I|)}|A_I|^{d - |I|}}{(n - |I|)^{d - |I|}} - 1 - (d - |I|)
\left(\frac{2^{|I|}|A_I|}{n-|I|} - 1\right)\right| \leq 
(d - |I|)^2\left(\frac{2^{|I|}|A_I|}{n-|I|} - 1\right)^2$$
Multiplying this equation by $\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!}$ and using Proposition 
\ref{exponentprop} with $x = |I|$ gives
\begin{align*}&\left|2^{-{{d - |I|} \choose 2}}\frac{|A_I|^{d - |I|}}{(d - |I|)!} - 
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!} - 
(d - |I|)\left(\frac{2^{|I|}|A_I|}{n-|I|} - 1\right)\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!}\right| \\
&= \left|2^{-{{d - |I|} \choose 2}}\frac{|A_I|^{d - |I|}}{(d - |I|)!} - 
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n - |I|)^{d-|I|}}{(d - |I|)!} - 
\left(A_I - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n - |I|)^{d-|I|-1}}{(d-|I|-1)!}\right| \\
&\leq (d - |I|)^2\left(\frac{2^{|I|}A_I}{n-|I|} - 1\right)^2\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!}\end{align*}
\end{proof}
\begin{lemma}\label{ndvpartthreelemma}
If $|A_I| > d - |I|$ then $\left|2^{-{{d - |I|} \choose 2}}{{|A_I|} \choose {d-|I|}} - 2^{-{{d - |I|} \choose 2}}
\frac{|A_I|^{d - |I|}}{(d - |I|)!}\right| \leq 2^{-{{d - |I|} \choose 2}}|A_I|^{d-|I|-1}$
\end{lemma}
\begin{proof}
Applying Proposition \ref{factorialapproxprop} on $|A_I|$ and $d - |I|$ gives 
$$\left|\frac{|A_I|^{d-|I|}}{(d-|I|)!} - {{|A_I|} \choose {d-|I|}}\right| \leq \frac{(d-|I|)^2}{2|A_I|}\frac{|A_I|^{d-|I|}}{(d-|I|)!} 
\leq |A_I|^{d-|I|-1}$$
Multiplying this equation by $2^{-{{d - |I|} \choose 2}}$ gives the claimed result.
\end{proof}
\begin{lemma}\label{ndvpartfourlemma}
For all $\epsilon_1 \in (0,1)$, if $|A_I| > {d^2}(2e - e\ln{\epsilon_1})(2e + 2 - e\ln{\epsilon_1})$ then 
$$P\left[\left|deg_G(I) - 2^{-{{d-|I|} \choose 2}}{|A_I| \choose {d-|I|}}\right| > 
e(2 - \ln{\epsilon_1})\frac{(d-|I|)^2}{(d-|I|)!}|A_I|^{d-|I|-1}\right] < \epsilon_1$$
\end{lemma}
\begin{proof}
This lemma follows immediately from applying Theorem \ref{cliqueboundtheoremone} on the random graph $G$ restricted to the vertices $A_I$.
\end{proof}
Combining Lemmas \ref{ndvpartonelemma}, \ref{ndvparttwolemma}, \ref{ndvpartthreelemma}, and \ref{ndvpartfourlemma}, we have that under 
the given conditions, 
\begin{align*}
P\Big(&\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| > \\
&2^{{{|I|} \choose 2} - {d \choose 2}}n^{d - |I| - 1} + (d - |I|)^2\left(\frac{2^{|I|}|A_I|}{n-|I|} - 1\right)^2
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!} + \\
&2^{-{{d - |I|} \choose 2}}|A_I|^{d-|I|-1} + e(2 - \ln{\epsilon_1})\frac{(d-|I|)^2}{(d-|I|)!}|A_I|^{d-|I|-1}\Big) < \epsilon_1
\end{align*}
The result now reduces to showing the following equation 
$$2^{{{|I|} \choose 2} - {d \choose 2}}n^{d - |I| - 1} + 
2^{-{{d - |I|} \choose 2}}|A_I|^{d-|I|-1} + e(2 - \ln{\epsilon_1})\frac{(d-|I|)^2}{(d-|I|)!}|A_I|^{d-|I|-1} \leq 
10(2 - \ln{\epsilon_1})n^{d-|I|-1}$$
which follows from the facts that $|I| < d$, $|A_I| \leq n$, and $\frac{(d-|I|)^2}{(d-|I|)!} \leq 2$.
\end{proof}
To use Lemma \ref{ndvavassumedlemma} to Prove Theorem \ref{cliqueboundtheoremtwo}, we need probabilistic bounds 
on $|A_I|$.
\begin{lemma}\label{avboundslemma}
For all $\epsilon_2 \in (0,1)$, $P\left[||A_I| - 2^{-|I|}(n - |I|)| > e(2 - \ln{\epsilon_2})\sqrt{n}\right] < \epsilon_2$
\end{lemma}
\begin{proof}
This will follow from the following lemma.
\begin{lemma}\label{randomvardeviationlemma}
If $x_1, \cdots, x_n$ are independent random variables such that for all $i$, $x_i \in [0,1]$, then 
for all $\epsilon_2 \in (0,1)$, 
$P\left[|\sum_{i=1}^{n}{x_i} - \sum_{i=1}^{n}{E[x_i]}| > e(2 - \ln{\epsilon_2})\sqrt{n}\right] < \epsilon_2$.
\end{lemma}
\begin{proof}
To prove this, we obtain probabilistic bounds on high powers of the quantity 
$\sum_{i=1}^{n}{(x_i - E[x_i])}$.
\begin{lemma}\label{randomvarpowercalculationlemma}
For all positive even $q$, $E\left[\left(\sum_{i=1}^{n}{(x_i - E[x_i])}\right)^q\right] \leq q!n^{\frac{q}{2}}$.
\end{lemma}
\begin{proof}
Note that 
$E\left[\left(\sum_{i=1}^{n}{(x_i - E[x_i])}\right)^q\right] = 
\sum_{i_1,\cdots,i_q \in [n]}{E\left[\prod_{j=1}^{q}{(x_{i_j} - E[x_{i_j}])}\right]}$

Every term in this sum has value less than $1$. Furthermore, for every nonzero term in this sum, 
no element of $\{i_1, \cdots, i_q\}$ can be unique, so this sum is at most the number of ordered multi-sets 
$\{i_1, \cdots i_q\}$ with elements in $[1,n-|I|]$ which have no unique elements. Thus, we just need to 
prove that this number is at most $q!n^{\frac{q}{2}}$, which follows immediately from the following lemma.
\begin{definition}
Let $f(k,n)$ be the number of ordered multi-sets $\{i_1, \cdots i_k\}$ with elements in $[n]$ which have no unique elements.
\end{definition}
\begin{lemma}\label{recursiveformulalemma}
For all $k,n$, $f(k,n) \leq k!{n^{\lfloor\frac{k}{2}\rfloor}}$.
\end{lemma}
\begin{proof}
We have the following recursive formula.
\begin{proposition}\label{recursiveformulaprop}
If $k \geq 2$ then $f(k,n) = n\sum_{j=1}^{k-1}{{{k-1} \choose {j}}f(k-j-1,n-1)}$
\end{proposition}
\begin{proof}
To see this, note that there are $n$ choices for $i_1$. Now for some $j \in [1,k-1]$, $j$ of the elements in 
$\{i_2, \cdots, i_k\}$ must be equal to $i_1$, and there are ${{k-1} \choose {j}}$ choices for these elements. 
Finally, once these elements have been chosen, the number of choices for the remaining elements is 
$f(k-j-1,n-1)$.
\end{proof}
We now prove Lemma \ref{recursiveformulalemma} by induction. 
If $k = 0$ then $f(n,k) = 1$. If $k = 1$ then $f(n,k) = 0$. If $k = 2$ then $f(k,n) = n$. If $k \geq 2$ 
then by the inductive hypothesis and Proposition \ref{recursiveformulaprop}, 
\begin{align*}
f(k,n) &= n\sum_{j=1}^{k-1}{{{k-1} \choose {j}}f(k-j-1,n-1)} \\
&\leq n\sum_{j=1}^{k-1}{{{k-1} \choose{j}}
(k-j-1)!{n^{\lfloor\frac{k-j-1}{2}\rfloor}}} = n(k-1)!\sum_{j=1}^{k-1}{\frac{1}{j!}{n^{\lfloor\frac{k-j-1}{2}\rfloor}}} \\
&\leq (e-1)n(k - 1)!{n^{\lfloor\frac{k}{2} - 1\rfloor}} < k!{n^{\lfloor\frac{k}{2}\rfloor}}
\end{align*}
This completes the proof of Lemma \ref{recursiveformulalemma} which in turn completes the proof of 
Lemma \ref{randomvarpowercalculationlemma}
\end{proof}
\end{proof}
We now prove Lemma \ref{randomvardeviationlemma}. Using Lemma \ref{randomvarpowercalculationlemma} and Markov's inequality, 
\begin{align*}
\epsilon_2 &> P\left[\left(\sum_{i=1}^{n}{(x_i - E[x_i])}\right)^q > 
\frac{E[\left(\sum_{i=1}^{n}{(x_i - E[x_i])}\right)^q]}{\epsilon_2}\right] \\
&\geq P\left[\left(\sum_{i=1}^{n}{(x_i - E[x_i])}\right)^q > \frac{q!n^{\frac{q}{2}}}{\epsilon_2}\right] 
\geq P\left[|\sum_{i=1}^{n}{x_i} - \sum_{i=1}^{n}{E[x_i]}| > \frac{q\sqrt{n}}{\sqrt[q]{\epsilon_2}}\right]
\end{align*}
Following similar logic as before, if we take $q$ to be the smallest even positive integer which is at least 
$-\ln{\epsilon_2}$ then $q < 2 + \ln{\epsilon_2}$ and $\frac{1}{\sqrt[q]{\epsilon_2}} \leq e$. Thus, 
$P\left[|\sum_{i=1}^{n}{x_i} - \sum_{i=1}^{n}{E[x_i]}| > e(2 - \ln{\epsilon_2})\sqrt{n}\right] < \epsilon_2$, as needed.
\end{proof}
We now use Lemma \ref{randomvardeviationlemma} to prove Lemma \ref{avboundslemma}.
If we let $x_i$ be $1$ if $i \notin I$ and $i$ is adjancent to all 
vertices in $I$ and $0$ otherwise then $\sum_{i=1}^{n}{x_i} = A_I$. The expected value of 
$A_I = \sum_{i=1}^{n}{x_i}$ is $2^{-|I|}(n - |I|)$, so applying Lemma \ref{randomvardeviationlemma}, for all 
$\epsilon_2 \in (0,1)$, $P\left[|A_I - 2^{-|I|}(n - |I|)| > e(2 - \ln{\epsilon_2})\sqrt{n}\right] < \epsilon_2$. 
\end{proof}
Now recall that by Lemma \ref{ndvavassumedlemma}, for any $\epsilon_1 \in (0,1)$, 
\begin{align*}
P\Big(&\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| > \\
&10(2 - \ln{\epsilon_1})n^{d-|I|-1} + (d - |I|)^2\left(\frac{2^{|I|}|A_I|}{n-|I|} - 1\right)^2
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!}\Big) < \epsilon_1
\end{align*} 
so long as the following conditions hold:
\begin{enumerate}
\item $(d - |I|)\left|\frac{2^{|I|}|A_I|}{n - |I|} - 1\right| \leq 1$
\item $|A_I| > {d^2}(2e - e\ln{\epsilon_1})(2e + 2 - e\ln{\epsilon_1})$
\end{enumerate}
Taking $\epsilon_1 = \epsilon_2 = \frac{\epsilon}{2}$, plugging Lemma \ref{avboundslemma} into these equations and using the 
union bound, we have that 
\begin{align*}
P\Big(&\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| > \\
&10(3 - \ln{\epsilon})n^{d-|I|-1} + (d - |I|)^2\left(\frac{2^{|I|}e(3 - \ln{\epsilon})\sqrt{n}}{n-|I|}\right)^2
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!}\Big) < \epsilon
\end{align*} 
so long as the corresponding conditions hold. Assuming these conditions hold for now, since $|I| < \frac{n}{16}$, $|I| < d$, 
$\frac{(d-|I|)^2}{(d - |I|)!} \leq 2$, and $2^{|I|}2^{{|I|} \choose 2} = 2^{{|I|+1} \choose 2}$,
\begin{align*}
(d - |I|)^2\left(\frac{2^{|I|}e(3 - \ln{\epsilon})\sqrt{n}}{n-|I|}\right)^2
\frac{2^{{{|I|} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|}}{(d - |I|)!} &\leq 
2\frac{2^{|I|}e^2(3 - \ln{\epsilon})^2{n}}{(n - |I|)}(n-|I|)^{d-|I|-1} \\
&< 10 \cdot {2^d}(3 - \ln{\epsilon})^2{n}^{d-|I|-1}
\end{align*}
Plugging this in we have that
\begin{align*}
P\Big(&\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}} - 
\left(|A_I| - \frac{n-|I|}{2^{|I|}}\right)\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!}\right| > \\
&2^{d+4}(3 - \ln{\epsilon})^2n^{d-|I|-1}\Big) < \epsilon
\end{align*}
as needed. For the first part of Theorem \ref{cliqueboundtheoremtwo}, note that this implies that 
\begin{align*}
P\Big(&\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}}\right| > \\
&\left||A_I| - \frac{n-|I|}{2^{|I|}}\right|\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!} 
+ 2^{d+4}(3 - \ln{\epsilon})^2n^{d-|I|-1}\Big) < \epsilon
\end{align*}
Plugging in Lemma \ref{avboundslemma} and noting that
$$e(3 - \ln{\epsilon})\sqrt{n}\frac{2^{{{|I|+1} \choose 2} - {d \choose 2}}(n-|I|)^{d-|I|-1}}{(d-|I|-1)!} 
< 4(3 - \ln{\epsilon})n^{d - |I| - \frac{1}{2}}$$
we have that 
$$P\Big(\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}}\right| > 
4(3 - \ln{\epsilon})n^{d - |I| - \frac{1}{2}} + 2^{d+4}(3 - \ln{\epsilon})^2n^{d-|I|-1}\Big) < \epsilon$$
Since $n \geq 4{d^2}2^{2d}(3 - \ln{\epsilon})^2$ and $d \geq 2$, 
$$2^{d+4}(3 - \ln{\epsilon})^2{n}^{d-|I|-1} \leq 
4(3 - \ln{\epsilon})n^{d - |I| - \frac{1}{2}}$$
Plugging this in gives that 
$$P\Big(\left|deg_G(I) - 2^{{{|I|} \choose 2} - {d \choose 2}}{{n-|I|} \choose {d - |I|}}\right| > 
8(3 - \ln{\epsilon})n^{d - |I| - \frac{1}{2}}\Big) < \epsilon$$
as needed. All that is left is to check the conditions for Lemma \ref{ndvavassumedlemma}, which are as follows.
\begin{enumerate}
\item $(d - |I|)\frac{2^{|I|}e(3 - \ln{\epsilon})\sqrt{n}}{n-|I|} \leq 1$
\item $2^{-|I|}(n - |I|) > {d^2}e(3 - \ln{\epsilon})(3e + 2 - e\ln{\epsilon}) + e(3 - \ln{\epsilon})\sqrt{n}$
\end{enumerate}
These conditions are true if $n \geq 4{d^2}2^{2d}(3 - \ln{\epsilon})^2$. To see this, note that since $d > |I| > 0$ and  
$|I| < \frac{n}{16}$
\begin{enumerate}
\item $(d - |I|)2^{|I|}e(3 - \ln{\epsilon})\sqrt{n} \leq d2^{|I|}e(3 - \ln{\epsilon})\sqrt{n} - |I| 
\leq \frac{e}{4}\sqrt{4{d^2}2^{2d}(3 - \ln{\epsilon})^2}\sqrt{n} - |I| \leq n - |I|$
\item $2^{|I|}{d^2}e(3 - \ln{\epsilon})(3e + 2 - e\ln{\epsilon}) < 2^{|I|}{d^2}e^2\frac{3e + 2}{3e}(3 - \ln{\epsilon})^2 < 
10 \cdot {2^{|I|}}{d^2}(3 - \ln{\epsilon})^2 \leq \frac{5}{16}n$
\item $2^{|I|}e(3 - \ln{\epsilon})\sqrt{n} < 4 \cdot {2^{|I|}}(3 - \ln{\epsilon})\left(2d{2^{d}}(3 - \ln{\epsilon})\right) \leq \frac{n}{2}$
\end{enumerate}
Dividing the first statement by $n - |I|$ gives the first condition. Using the second and third statements, 
$$2^{|I|}{d^2}e(3 - \ln{\epsilon})(3e + 2 - e\ln{\epsilon}) + 2^{|I|}e(3 - \ln{\epsilon})\sqrt{n} < \frac{13}{16}n < n - |I|$$
Dividing this by $2^{|I|}$ gives the second condition, as needed.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "stoc"
%%% End: 


==> previouspsdproof.tex <==
\section{PSD'ness of the expectation matrix}\label{sec:psdexpectation}
As first steps and as a warmup for the final proof we first show that the expectation matrix $\ex[\mm]$ is PSD. We start by writing down $E \equiv \ex[\mm]$.

\begin{claim}
For $I,J \in \bnlr$, and $E \equiv \ex[\mm]$, 
\begin{equation}
  \label{eq:exm}
  E(I,J) = \binom{n-|I\cup J|}{2r-|I \cup J|} \cdot \frac{\binom{k}{|I \cup J|}}{\binom{2r}{|I\cup J|}} \cdot 2^{-\binom{2r}{2}}.
\end{equation}
\end{claim}
\begin{proof}
 The claim follows from observing that for any set $K$, $\ex[deg_G(K)] = \binom{n-|I|}{2r-|I|} \cdot 2^{-\binom{2r}{2}}$. For, all $K$, there are $\binom{n-|K|}{2r-|K|}$ sets of size $2r$ containing $K$, and each is a clique with probability $2^{-\binom{2r}{2}}$. 
\end{proof}

Note that, the expectation matrix above is just a scalar multiple of $\m_{Gr}$ (viewed as a matrix) as defined in \eref{eq:grigoriev}. Therefore, by \tref{th:grigknapsack}, $E$ as defined above is PSD for $r < k$. We give a simpler proof of this claim here. We then build on these ideas to get lower bounds not only for the least eigenvalue of $E$, but for all of them, which will be critical for what follows. 

The main claim of the section is the following.
\begin{theorem}\label{th:knapsack}
The matrix $E$ is PSD for $r < \min(k,n-k)$.   
\end{theorem}

As $E$ is singular, one needs to exhibit extra care while trying to show $E$ is PSD. Fortunately, the kernel of $E$ has a simple structure and we exploit this. The next lemma is proved in \cite{GrigorievHP02}, and we repeat the simple proof here as we will also use a similar argument later.
\begin{lemma}\label{lm:kernelE}
  The kernel of $E$ has dimension at least $\sum_{i=0}^{r-1} \binom{n}{i}$. 
\end{lemma}
\begin{proof}
  For any $J \subseteq [n]$, $|J| < r$, let $f_J \in \reals^{\bnlr}$ be the vector defined by
  \begin{align*}
 f_J(K) =    \begin{cases}
      1 &\text{$K = J \cup \{j\}$, $j \notin J$}\\
 (|J|-k) & K = J\\
0 &\text{otherwise}
    \end{cases}.
  \end{align*}
We claim that the vectors $\{f_J: J \subseteq [n], |J| < r\}$ are (1) in the kernel of $E$ and (2) are linearly independent.

Proof of (1): For any $f_J$ and $K$, $|K| \leq r$, 
\begin{align*}
  (E\cdot f_J)(I) &= \sum_{K: |K| \leq r} E(I,K) f_J(K) = (|J| - k) E(I,J) + \sum_{j \notin J} E(I,J \cup \{j\})\\
&= (|J| - k) E(I,J) + \sum_{j \in I\setminus J} E(I,J) + \sum_{j \notin (I \cup J)}E(I,J \cup \{j\})\\
&\comm \text{\hspace*{.2in} (E(I,J) only depends on $I \cup J$.)}\\
&= (|I \cup J| - k) E\bkets{X_{I \cup J}} + \sum_{j \notin (I \cup J)} E\bkets{x_j \cdot X_{I \cup J}},
\end{align*}
where in the last equation we used the interpretation of $E$ as a linear mapping. It now follows that $f_J$ is in the kernel as, $E$ satisfies the relation
\begin{align*}
  0 &= E\bkets{\bkets{\sum_i x_i -k}X_{I\cup J}} = \sum_i E\bkets{x_i X_{I\cup J}} - k E\bkets{X_{I\cup J}}\\
&= \bkets{|I\cup J|-k} E\bkets{X_{I\cup J}} + \sum_{j \notin I} E\bkets{X_{I \cup J \cup {j}}}.
\end{align*}

Proof of (2): Look at the vectors $((f_I))$ in decreasing order of the sizes $|I|$. Then, each vector $f_I$ introduces a new non-zero coordinate, $f_I(I)$, that was not covered before. Thus the collection of vectors is linearly independent.
\end{proof}
  
Now that we have a handle on the kernel of $E$, we use a trick due to Laurent \cite{Laurent03} to show PSD'ness of $E$. Let $E_r$ be the principal sub-matrix of $E$ corresponding to the subsets of size exactly $r$. We will show that $E_r$ is positive definite and conclude that $E$ is PSD by appealing to the interlacing eigenvalues theorem, \lref{lm:interlacing}. Technically, the proof of the next lemma is where we differ in the proof \tref{th:knapsack} from similar claims in \cite{Laurent03}, \cite{GrigorievHP02} who use various results about hyper-geometric series.
\begin{lemma}\label{lm:erpd}
For $r < \min(k,n-k)$, the matrix $E_r$ is positive definite. 
\end{lemma}
\begin{proof}
We will show this by writing $E_r$ as a suitable positive linear combination of the PSD matrices $P_t$'s from \sref{sec:prelims}. More concretely, for any $\alpha_0,\ldots,\alpha_t > 0$, we have
$$ 0 \prec \sum_t \alpha_t P_t = \sum_{\ell = 0}^r \bkets{\sum_{t=0}^\ell \alpha_t \binom{\ell}{t}} D_\ell.$$
Now, let $e_\ell = E(X(I))$ for any $I$, $|I| = 2r-\ell$, i.e.,
$$e_\ell = 2^{-\binom{2r}{2}} \cdot \binom{n-2r+\ell}{d-2r+\ell} \cdot \frac{\binom{k}{2r-\ell}}{\binom{d}{2r-\ell}}.$$
Then, $E = \sum_{\ell = 0}^r e_\ell D_\ell$. Therefore, we will be done if we can find $\alpha_t$'s such that for every $0 \leq \ell \leq r$, $ e_\ell = \sum_{t=0}^\ell \alpha_t \binom{\ell}{t}$. By examining the first values of $\ell$, it is easy to guess what the $\alpha_t$ should be. 
\Anote{There was a calculation error below. I changed the value of $\alpha_t$ (there was a redundant "-1") and it now seems to check}
First observe that $e_\ell = e_0 \cdot \binom{n-2r+\ell}{\ell}/\binom{k-2r+\ell}{\ell}$ and let $\alpha_t = e_0 \binom{n-k}{t}/\binom{k-2r+t}{t}$. Then,
\begin{align*}
 e_0 \binom{n-2r+\ell}{\ell} &= e_0 \sum_{t=0}^\ell \binom{n-k}{t} \cdot \binom{k-2r+\ell}{\ell-t}\\
&= \sum_{t=0}^\ell  \alpha_t \cdot \binom{k-2r+t}{t} \binom{k-2r+\ell}{\ell-t}\\
&= \sum_{t=0}^\ell \alpha_t \cdot \binom{\ell}{t} \cdot \binom{k-2r+\ell}{\ell}.
\end{align*}
Therefore, $e_\ell = \sum_t \binom{\ell}{t} \alpha_t$ and the lemma now follows:
\begin{align*}
  E_r = \sum_{\ell = 0}^r e_\ell D_\ell = \sum_{\ell =0}^r \left(\sum_{t=0}^\ell \alpha_t \binom{\ell}{t}\right) D_\ell  \succeq \alpha_r \mathds{I}.
\end{align*}
\end{proof}


\begin{proof}[Proof of \tref{th:knapsack}]
From the previous claim and \lref{lm:interlacing}, $E$ has at least $\binom{n}{r}$ eigenvalues which are positive. The claim now follows by \lref{lm:kernelE}.
\end{proof}

\section{PSD'ness of dual certificate}\label{sec:psdmaintech}
We are now ready to prove our main result, \tref{th:main}, by showing that the mapping $\mm$ will be PSD with high probability (\tref{th:mainpsd}). 

As it turns out, the matrix $\mm$ is a little unwieldy because of high variance entries. We will instead work with a new matrix $\mm'_r$ such that $\mm'_r \succeq 0$ implies $\mm$ is PSD. We then show PSD'ness of $\mm'_r$ by applying the high-level approach from the introduction to $\mm'_r$ (instead of $\mm$ as sketched originally).

In \sref{sec:reduction} we define our main object, the matrix $\mm'_r$, a variant of the principal minor of $\mm$ corresponding to subsets of size exactly $r$. In \sref{sec:psdmmr} we show that $\mm_r'$ is PSD. In \sref{sec:localrand} we develop some combinatorial techniques which help us estimate norms of locally random matrices. We put all the pieces together to show the PSD'ness of dual certificate in \sref{sec:wrapup}. 

%We first describe this reduction and then prove PSD'ness of $\mm'_r$ in the following sections by applying the high-level approach from the introduction to $\mm'_r$ (instead of $\mm$ as sketched).

\subsection{Reduction to positive definiteness of $\mm_r'$}\label{sec:reduction}
As was done in \sref{sec:psdexpectation}, we will lower bound the dimension of kernel of $\mm$ and then find a large principal submatrix which is positive definite. To this end, let $\mm_r$ be the principal submatrix of $\mm$ corresponding to the rows and columns of size exactly $r$.   

We shall use the following notations for brevity: For any set $I \subseteq [n]$, let $\mathcal{E}(I) = \{\{i,j\}: i\neq j \in I\}$. For $0 \leq i \leq r$, let $k(i) = \binom{k}{2r-i}/\binom{2r}{2r-i}$. 

A problem with the matrix $M_r$ is that the diagonal entries have very large variance: The expected value of each diagonal entry is roughly $\Theta_r(n^r k^r)$. However, with probability $\Theta_r(1)$, the actual entry will be zero (if the corresponding set is not a clique) which in turn will also lead to the entire row and column being zero as well. This leads to strong technical difficulties. To overcome this, we study a closely related matrix which does not have the same variance issues.

For every $T \subseteq [n]$, let $M_T \in \reals^{\binom{[n]}{r} \times \binom{[n]}{r}}$, with $M_T(I,J) = k(|I \cap J|)$ if $I \cup J \subseteq T$, and $G$ contains every edge in $\mathcal{E}(T) \setminus \mathcal{E}(I) \cup \mathcal{E}(J)$ (i.e., the only edges in $T$ missing in $G$ are those with both end points in one of $I$ or $J$). We will study the matrix 
\begin{equation}\label{eq:mr}  
M'_r = \sum_{T: |T| = 2r} M_T.
\end{equation}

Intuitively, for every $I,J$, $M_r'(I,J)$  is what $M(I,J)$ would be had we added cliques on the subsets $I$, $J$ to the graph. The above definition avoids the problem of the whole row and column corresponding to $I$ or $J$ becoming zero if either was not a clique, and controls the variance.

We now reduce PSD'ness of $M$ to that of $M_r'$. 
\begin{lemma}
  For any graph $G$, the kernel of $\mm_G$ has dimension at least $\sum_{\ell = 0}^{r-1} \binom{n}{\ell} + |\{I: |I| = r, \text{$I$ not a clique in $G$}\}|$. 
\end{lemma}
Compared to \lref{lm:kernelE}, the difference is the last additive term. 
\begin{proof}
  The same proof as in \lref{lm:kernelE} shows that the vectors $\{f_J: |J| < r\}$ defined there also lie in the kernel of $\mm_G$. The reason is that the proof of \lref{lm:kernelE} only relied on the equations defining the dual certificate - last equation in \ref{eq:dualcert}, which $\mm_G$ also satisfies.

Let $N = \sum_\ell^r \binom{n}{\ell}$ and for a set $I$, let $e_I \in \reals^N$ be the vector with $1$ in the $I$'th coordinate and $0$'s elsewhere. Observe that if a set $I$, $|I| \leq r$, is not a clique then, the $I$'th row and $I$'th column of $\mm_G$ are identically zero. Therefore, for every such vector $I$, $e_I$ is in the kernel of $\mm_G$. 

Let $V = \{f_J: |J| < r\} \cup \{e_J: |J| = r, \text{$J$ not a clique in $G$}\}$. We claim that the vectors in $V$ are linearly independent. Look at the vectors in $V$ in decreasing order of the sizes $|I|$. Then, each vector $f \in V$ introduces a new non-zero coordinate (corresponding to the set describing $f$) that was not covered before. Thus the collection of vectors is linearly independent.
\end{proof}

\begin{lemma}\label{lm:subtofull}
  If $M_r'$ is positive definite, then the mapping $\mm$ is PSD. 
\end{lemma}
\begin{proof}
First note that, for any $I,J$, $M_r(I,J) = M_r'(I,J)$ if $I$ and $J$ are cliques in $G$ and $M_r(I,J) = 0$ otherwise. For, suppose that $I$ and $J$ are cliques in $G$. Then, $M_T(I,J) = k(|I \cap J|)$ if $I \cup J \subseteq T$ and $T$ is a clique and $0$ otherwise. Therefore, 
$$M_r'(I,J) = \sum_{T} M_T(I,J) = k(|I \cap J|)\cdot \left|\{T: I \cup J \subseteq T, T \text{ clique}\}\right| = M_r(I,J).$$

Therefore, the principal submatrix of $M_r$ corresponding to cliques of size exactly $r$ is the same as in $M_r'$ and hence is positive definite by the assumption. Thus, if we let $N_r$ be the number of cliques of size exactly $r$ in $G$, then by \lref{lm:interlacing}, $M_r$ and hence $M$, has at least $N_r$ positive eigenvalues. The claim now follows from the fact that the kernel has dimension at least $\sum_{\ell=0}^r \binom{n}{\ell} - N_r$ by the previous lemma. 
\end{proof}

%We next prove \lref{lm:maintech}.
\subsection{Positive definiteness of $\mm_r'$}\label{sec:psdmmr}
We now show that the matrix $M_r'$ defined in the last section is positive definite with high probability. 
\begin{lemma}[Main Technical Lemma]\label{lm:maintech}
For $c$ a sufficiently large constant the following holds. The matrix $M_r' \in \reals^{\binom{[n]}{r} \times \binom{[n]}{r}}$ defined by \eref{eq:mr} is positive definite with high probability, for $k < 2^{-cr} (\sqrt{n}/\log n)^{1/r}$.
\end{lemma}

For the remainder of this section, we shall use the following additional notations: 
\begin{itemize}
\item For $0 \leq i \leq r$, let 
$$\alpha(i) = k(i) \cdot \binom{n-2r+i}{i} \cdot 2^{-\binom{2r}{2} + 2 \binom{r}{2} - \binom{r-i}{2}} = k(i) \cdot \binom{n-2r+i}{i} \cdot 2^{-r^2 - \binom{i}{2}}.$$
\item For $0 \leq i \leq r$, let 
$$k'(i) = k(i)/2^{r^2 + \binom{i}{2}} = \binom{k}{2r-i}/\binom{2r}{2r-i} \cdot 2^{r^2 + \binom{i}{2}}.$$ 
\item For $0 \leq i \leq r$, let $p(i) = 2^{-(r-i)^2}$. Then, for $I,J \in \bnr$ with $|I \cap J| = i$, $p(i)$ is the probability that $\mathcal{E}(I \cup J) \setminus (\mathcal{E}(I) \cup \mathcal{E}(J)) \subseteq G$.
\item In the following we will adopt the convention that $I,J,K$ denote elements of $\binom{[n]}{r}$ and $T,T'$ denote elements of $\binom{[n]}{2r}$. 
\item All matrices considered below will be over $\reals^{\binom{[n]}{r} \times \binom{[n]}{r}}$ unless otherwise specified.
\item We write $A \approx_r B$ if there exist constants $c, C$ such that $c^{r^2} B \leq A \leq C^{r^2} B$.
\end{itemize}

For the proof of \lref{lm:maintech} we decompose the matrix $M_r'$ as $M_r' = E + L + \Delta$, where (a) $E = \ex[M_r']$ is the expectation matrix; (b) $L$ will be a ``local'' random matrix such that for sets $I,J$, $L(I,J)$ only depends on the edges between the vertices of $I \cup J$ and (c) $\Delta$ is a ``global'' error matrix whose entries are small in magnitude.

To this end, first observe that by \eref{eq:mr}, for $E \equiv \ex[M_r']$, 
\begin{equation}
  \label{eq:Evalue}
  E(I,J) = \alpha(|I \cap J|).
\end{equation}
This is because there are $\binom{n-|I \cup J|}{2r-|I \cup J|}$ many sets $T$ of size $2r$ that contain $I,J$ and every such $T$ contributes to $M_r'(I,J)$ by an additive $k(|I \cap J|)$ amount with probability $2^{-r^2 - \binom{i}{2}}$. 

Now, define $L \in \rnr$ as follows: for $I,J \in \bnr$,
\begin{equation}
  \label{eq:defL}
L(I,J) =
\begin{cases}
 \alpha(|I \cap J|) \cdot \frac{1-p(|I \cap J|)}{p(|I \cap J|)} &\text{ if $\mathcal{E}(I \cup J) \setminus (\mathcal{E}(I) \cup \mathcal{E}(J)) \subseteq G$}\\
- \alpha(|I \cap J|) &\text{otherwise}
\end{cases}.
\end{equation}
Finally, define $\Delta = M_r' - E - L$. The proof proceeds in three modular steps:
\begin{enumerate}
\item We use the results from \sref{sec:jscheme} to show that $E \succ 0$ and has a large least eigenvalue (roughly $\Omega_r(k^r n^r)$).
\item We next show that $\|L\| \ll k^{2r} n^{r-1/2}$ by exploiting the recursive structure of the matrix $L$ and some careful trace calculations. This is the most technically intensive part of the proof. 
\item We then show that $\|\Delta\| \ll k^{2r} n^{r-1/2}$. This is done by first showing that each entry of $\Delta$ is small in magnitude and using \lref{lm:Gershgorin}.
\end{enumerate}

The next three subsections address the three steps.
\subsubsection{Estimating the eigenvalues of the expectation matrix}\label{sec:expectation}
We now estimate the spectrum of $E[M_r']$. In the following, we recall the notation from \lref{lm:eigenschemes}. 

\begin{lemma}\label{lm:exspectrum}
If $k < n/2^{cr^2}$ for a sufficiently large constant $c$, then, for $0 \leq j \leq r$,  $\lambda_j(\ex[M_r']) \geq k^{2r-j} n^r/2^{O(r^2)}$.
\end{lemma}
\begin{proof}
From the definition of $E$ and \eref{eq:Evalue}, $E = \sum_\ell \alpha(\ell) D_\ell$, where $\alpha(\ell) \approx_r k^{2r-\ell} n^{\ell}$. We next express $Q$ as a linear combination of $P_t$'s: $Q = \sum_t \beta_t P_t$. Then, by \clref{clm:dtop},
$$\beta_t = \sum_{\ell \leq t} (-1)^{t-\ell} \binom{t}{\ell} \alpha(\ell).$$
Now, if $k < n/2^{O(r^2)}$ for a sufficiently big constant, then $\alpha(\ell)$'s increase geometrically and the above sum will be dominated by the last term so that $\beta_t \geq \alpha_t/2 \approx_r k^{2r-t} n^t$. Therefore, by \lref{lm:eigenschemes} and the fact that $P_t$'s are PSD,
 \begin{align*}
   \lambda_j(Q) &= \sum_t \beta_t \lambda_j(P_t) = \sum_{t \geq j} \beta_t \binom{n-t-j}{r-t} \binom{r-t}{t-j}\\
&\geq 2^{-O(r^2)} \sum_{t \geq j} k^{2r-\ell} n^t \cdot n^{r-t} \geq k^{2r-j} n^r/2^{O(r^2)}.
 \end{align*}
\end{proof}

\subsubsection{Bounding the norm of the locally random matrix $L$}\label{sec:normboundL}
We next bound the norm of the matrix $L$.

\begin{lemma}\label{lm:Lnorm}
For some constant $C > 0$, with probability at least $1 - 1/n$ over the random graph $G$, 
$$\|L\| \leq O(1) \cdot 2^{C r^2} \cdot k^{2r} \cdot n^r \cdot \frac{\log n}{\sqrt{n}}.$$
\end{lemma}

We will prove the lemma by further decomposing $L$ according to the intersection sizes of the indexing sets and using the recursive structure of the matrix $M_r'$. For a matrix $X \in \reals^{\binom{[n]}{r_1} \times \binom{[n]}{r_2}}$, and $0 \leq i \leq \min{\{r_1,r_2\}}$, let $X^i \in \reals^{\binom{[n]}{r_1} \times \binom{[n]}{r_2}}$ be the matrix such that $X^i(I,J) = X(I,J)$ if $|I \cap J| = i$ and $0$ otherwise. The following claim immediately implies \lref{lm:Lnorm} as $L = \sum_{i=0}^r L^i$.

\begin{remark}
For this paper, we will only use the case where $r_1 = r_2 = r$. We put in this extra generality with an eye towards future work.
\end{remark}
\begin{claim}\label{clm:Lnorm1}
For some constant $C > 0$, with probability at least $1-1/n^2$ over the random graph $G$, for every $0 \leq i \leq r$, 
$$\|L^i\| \leq O(1) \cdot 2^{C r^2} \cdot k^{2r-i} \cdot n^{r} \cdot \frac{\log n}{\sqrt{n}}.$$
\end{claim}
We prove the claim by first studying the case $i=0$ (in a slightly more general setting) by some explicit trace calculations. We then use the recursive struture of the matrix $L$ to prove it for $i \geq 1$. We shall use the following notation.

For a matrix $X \in \reals^{\binom{[n]}{r_1-i} \times \binom{[n]}{r_2-i}}$, let $X^{(i)} \in \reals^{\binom{[n]}{r_1} \times \binom{[n]}{r_2}}$, be defined as follows:
\begin{equation}
  \label{eq:defextension}
  X^{(i)}(I,J) =
  \begin{cases}
X(I\setminus (I \cap J), J \setminus (I \cap J)) &\text{ if $|I \cap J| = i$}\\
0 &\text{ otherwise}
  \end{cases}.
\end{equation}

Finally, we define a sequence of matrices which are similar to $L^0$ for varying sizes of the indexing sets. For $a \in [r]$, let $R_a \in \reals^{\binom{n}{a} \times \binom{n}{a}}$ be the matrix defined as follows: for $V,W \in \binom{[n]}{a}$, 
\begin{equation}
  \label{eq:defR}
  R_a(V,W) =
  \begin{cases}
    2^{a^2} - 1 &\text{ if $V \cap W = \emptyset$ and $\{\{v,w\}: v \in V, w \in W\} \subseteq G$}\\
    -1 &\text{ if $V \cap W = \emptyset$ and $\{\{v,w\}: v \in V, w \in W\} \not\subseteq G$}\\
0 &\text{ if $V \cap W \neq \emptyset$} 
  \end{cases}.
\end{equation}

The following technical claim proved in Section \ref{sec:localrand} bounds the norm of $R_a$. The proof relies on computing the trace of powers of $R_a$. 
\begin{claim}[See Section \ref{sec:localrand}]\label{clm:maintechnicalL}
For some constant $C > 0$, for all $\epsilon \in (0,1)$,
$$\pr\left[ \|R_a\| > C 2^{a^2} \cdot \log(n/\epsilon) \cdot n^{a-1/2}\right] < \epsilon.$$ 
\end{claim}
Note that $2^{a^2} n^a$ is an easy bound for $\|R_a\|$ (each entry of the matrix is at most $2^{a^2}$ in magnitude); the main advantage of the claim is the multiplicative $n^{-1/2}$ factor. We shall also need the following lemma which allows us to exploit the recursive structure of our matrices.

\begin{lemma}\label{lm:recursiveL}
For $0 \leq i \leq \min{\{r_1,r_2\}}$ and $R \in \reals^{\binom{[n]}{r_1-i} \times \binom{[n]}{r_2-i}}$, if 
$R = R^0$ then $\|R^{(i)}\| \leq \binom{r_1}{i}\binom{r_2}{i} \cdot \|R\|$
\end{lemma}
\begin{proof}
We partition the entries of $R^{(i)}$ as follows. 
\begin{definition}
For any $X,Y,K$ such that $X \subseteq [1,r_1]$, $Y \subseteq [1,r_2]$, and $K \subseteq V(G)$ where $|K| = |X| = |Y| = i$, 
let $R_{X,Y,K}^{(i)}$ be the matrix such that the following is true: 
\begin{enumerate}
\item $R_{X,Y,K}^{(i)}(I,J) = R^{(i)}(I,J) = R(I \setminus K, J \setminus K)$ if 
$K = \{i_x: x \in X\} = \{j_y: y \in Y\}$ where $i_1, \cdots, i_{r_1}$ are the elements of $I$ in increasing order and $j_1, \cdots, j_{r_2}$ are the elements of $J$ in increasing order.
\item $R_{X,Y,K}^{(i)}(I,J) = 0$ otherwise.
\end{enumerate}
\end{definition}
\begin{proposition}\label{decompositionpropone}
For all $X,Y,K$, $||R_{X,Y,K}^{(i)}|| \leq ||R||$
\end{proposition}
\begin{proof}
The nonzero part of $R_{X,Y,K}^{(i)}$ can be viewed as a submatrix of $R$, so it cannot have 
larger induced norm than $R$.
\end{proof}
\begin{proposition}\label{decompositionproptwo}
$R^{(i)} = \sum_{X,Y,K}{R_{X,Y,K}^{(i)}}$
\end{proposition}
\begin{proof}
If $R^{(i)}(I,J) = 0$ then $\sum_{X,Y,K}{R_{X,Y,K}^{(i)}(I,J)} = 0$. If $R^{(i)}(I,J) \neq 0$ then 
$|I \cap J| = i$. This implies that $K = \{i_x: x \in X\} = \{j_y: y \in Y\}$ if and only if 
$K = I \cap J$, $X$ is the set of indices of $K$ in $I$, and $Y$ is the set of indices of $K$ in $J$, which 
happens for precisely one $X,Y,K$. Thus, $R_{X,Y,K}^{(i)}(I,J) = R^{(i)}(I,J)$ for precisely one $I,J,X$ 
and is $0$ otherwise, so $R^{(i)} = \sum_{X,Y,K}{R_{X,Y,K}^{(i)}}$, as needed.
\end{proof}
\begin{corollary}\label{decompositioncorone}
$||R^{(i)}|| \leq \sum_{X,Y}{||\sum_{K}{R_{X,Y,K}^{(i)}}||}$
\end{corollary}
\begin{proposition}\label{decompositionpropthree}
If $K_1$,$K_2$ are distinct subsets of $V(G)$ of size $x$, $R_{X,Y,K_1}^{(i)}(I_1,J_1) \neq 0$, and 
$R_{X,Y,K_2}^{(i)}(I_2,J_2) \neq 0$ then $I_1 \neq I_2$ and $J_1 \neq J_2$.
\end{proposition}
\begin{proof}
Assume that $I_1 = I_2 = I$ and let $i_1, \cdots, i_{r_1}$ be the elements of $I$ in increasing order. Then 
$K_1 = \{i_x: x \in X\} = K_2$. Contradiction. Following similar logic, we cannot have that $J_1 = J_2$ either. 
\end{proof}
\begin{corollary}\label{decompositioncortwo}
For any $X,Y \subseteq [1,n]$ of size $x$, $||\sum_{K}{R_{X,Y,K}^{(i)}}|| \leq ||R||$
\end{corollary}
\begin{proof}
Note that we can permute the rows and columns of a matrix without affecting its induced norm. By Proposition 
\ref{decompositionpropthree}, we can permute the rows and columns of $\sum_{K}{R_{X,Y,K}^{(i)}}$ to put it into block 
form where each block is the nonzero part of $R_{X,Y,K}^{(i)}$ for some $K$. For a matrix in block form, its norm is 
the maximum of the norms of the individual blocks, which by Proposition \ref{decompositionpropone} is at most $||R||$, as needed.
\end{proof}
With these results, Lemma \ref{lm:recursiveL} follows immediately. Plugging in Corollary \ref{decompositioncortwo} to 
Corollary \ref{decompositioncorone} gives 
$||R^{(i)}|| \leq \sum_{X,Y}{||\sum_{K}{R_{X,Y,K}^{(i)}}||} \leq \sum_{X,Y}{||R||} \leq 
{{r_1} \choose i}{{r_2} \choose i}||R||$, as needed.
\end{proof}

We now use the above statements to prove \clref{clm:Lnorm1} which in turn implies \lref{lm:Lnorm}.
\begin{proof}[Proof of \clref{clm:Lnorm1}]
We claim that for $0 \leq i \leq r$, 
\begin{equation}
  \label{eq:Lnorm11}
L^i = \alpha_i \cdot R_{r-i}^{(i)}.  
\end{equation}

To see the above, fix $I, J \in \bnr$ with $|I \cap J| = i$ and let $V = I \setminus (I \cap J)$, $W = J \setminus (I \cap J)$. Observe that 
$$\mathcal{E}(I \cup J) \setminus (\mathcal{E}(I) \cup \mathcal{E}(J)) = \{\{v,w\}: v \in V, w \in W\}.$$

We cosider two cases as in the definition of $L$. 

{\bf Case 1}. $\mathcal{E}(I \cup J) \setminus (\mathcal{E}(I) \cup \mathcal{E}(J)) \subseteq G$. Then, $R_{r-i}^{(i)}(I,J) = R_{r-i}(V,W) = 2^{(r-i)^2 - 1} = (1-p(i))/p(i)$. \eref{eq:Lnorm11} now follows from the first case of the definition of $L$.

{\bf Case 2}. $\mathcal{E}(I \cup J) \setminus (\mathcal{E}(I) \cup \mathcal{E}(J)) \not\subseteq G$. Then, $R_{r-i}^{(i)}(I,J) = R_{r-i}(V, W) = -1$. \eref{eq:Lnorm11} now follows from the second case of the definition of $L$. 

The claim now follows from \eref{eq:Lnorm11}, Claims \ref{clm:maintechnicalL}, and Lemma \ref{lm:recursiveL}.   
\end{proof}

\subsubsection{Bounding the norm of the global error matrix $\Delta$}\label{sec:normboundDelta}
The main claim of this section is the following bound on the spectral norm of $\Delta$.
\begin{lemma}\label{lm:Deltanorm}
For $n > C 2^{4r^2}$, with probability at least $1 - 1/n$ over the random graph $G$, 
$$\|\Delta\| \leq 2^{Cr^2} \cdot k^{2r} \cdot n^r \cdot \frac{\log n}{\sqrt{n}}.$$
\end{lemma}

The proof relies on the following bound on the individual entries of $\Delta$. 
\begin{lemma}\label{lm:Deltaentrywise}
For some universal constant $C$, and $n > C 2^{4r^2}$, with probability at least $1 - 1/n$ over the random graph $G$, for all $I,J \in \bnr$, with $i = |I \cap J|$,
$$|\Delta(I,J)| \leq 2^{C r^2} \cdot k^{2r-i} \cdot n^i \cdot \frac{\log n}{\sqrt{n}}.$$
\end{lemma}
Before proving the lemma, we first use it to bound $\|\Delta\|$.
\begin{proof}[Proof of \lref{lm:Deltanorm}]
Suppose that the conclusion of the previous lemma holds. Then, for any $I \in \bnr$,
\begin{align*}
\|\Delta \|\leq  \sum_J |\Delta(I,J)| &= \sum_{i=0}^r \sum_{J: | I \cap J| = i} |\Delta(I,J)|\\
&\leq \frac{2^{C r^2} k^{2r} (\log n)}{\sqrt{n}} \sum_{i=0}^r \sum_{J: |I \cap J| = i} (n/k)^i\\
&\leq \frac{ 2^{Cr^2} k^{2r} (\log n)}{\sqrt{n}} \sum_{i=0}^r (n/k)^i\,2^r n^{r-i}\\
&\leq \frac{ 2^{Cr^2} k^{2r} (\log n) n^r}{\sqrt{n}}.
\end{align*}
The lemma now follows from the above bound and \lref{lm:Gershgorin}.
\end{proof}

\begin{proof}[Proof of \lref{lm:Deltaentrywise}]
Fix sets $I,J$ with $|I \cap J| = i$. Let $\mathcal{A}$ be the event that $\mathcal{E}(I \cup J) \setminus (\mathcal{E}(I) \cup \mathcal{E}(J)) \subseteq G$. 

Then, by the second case of \eref{eq:defL}, conditioned on $\neg\mathcal{A}$ we have $\Delta(I,J) = 0$. Thus, the claim holds trivially in this case. In the following we condition on $\mathcal{A}$. Observe that
$$\ex[M_r'(I,J) \mid \mathcal{A}] = E(I,J)/\pr[\mathcal{A}] = E(I,J)/p(i).$$

We next use the following claim that $\deg_G(I\cup J)$ is concentrated around its mean when conditioned on $I \cup J$ being a clique. At a high level, this follows from the fact that conditioned on $I \cup J$ being a clique, $\deg_G(I \cup J)$ can be written as a (structured) low-degree polynomial in the indicator variables of the edges not in $I \cup J$ with small variance. We defer the proof to the appendix.

\begin{claim}[See Theorem \ref{cliqueboundtheoremtwo} of the appendix]\label{clm:degreebound}
For some constant $C > 0$,
$$\pr\left[\left| \deg_G(I \cup J) - 2^{-\binom{2r}{2} + \binom{2r-i}{2}} \cdot \binom{n-2r+i}{i}  \right| > C 2^{2r^2} \log(1/\epsilon) n^{i-1/2} \mid (I \cup J \text{ a clique})\right] < \epsilon.$$
\end{claim}


As a consequence of the above claim we also get concentration for $M_r'(I,J) \mid \mathcal{A}$. This is because $M_r'(I,J) \mid \mathcal{A}$ is identically distributed as $M(I,J) \mid (I \cup J\text{ a clique})$. Therefore, taking $\epsilon = 1/n^{2r+1}$ and applying a union bound over all sets $I,J$ we get that with probability at least $1-1/n$, for all $I,J$ such that $\mathcal{E}(I \cup J) \setminus (\mathcal{E}(I) \cup \mathcal{E}(J)) \subseteq G$, and $|I \cap J| = i$,

$$\left| M_r'(I,J) - k(i) 2^{-\binom{2r}{2} + \binom{2r-i}{2}} \cdot \binom{n-2r+i}{i} \right| < C r 2^{2r^2} \cdot k^{2r-i} \cdot (\log n) \cdot n^{i-1/2}.$$

Finally, observe that 
$$k(i) 2^{-\binom{2r}{2} + \binom{2r-i}{2}} \cdot \binom{n-2r+i}{i} = \alpha(i)/p(i),$$
and conditioned on $\mathcal{A}$, $\Delta(I,J) = M_r'(I,J) - \alpha(|I \cap J|)/p(|I \cap J|)$.  The lemma now follows by combining the above two bounds.
\end{proof}

\subsubsection{PSD'ness of $M_r'$}
We now prove \lref{lm:maintech}
\begin{proof}[Proof of \lref{lm:maintech}]
By \lref{lm:exspectrum}, we have that $E \succeq 2^{-Cr^2} k^r n^r \mathbb{I}$. Therefore, by \lref{lm:Lnorm} and \lref{lm:Deltanorm}, with probability at least $1-2/n$, the least eigenvalue of $M_r'$ is at least
$$2^{-Cr^2} k^r n^r - 2^{O(r^2)} k^{2r} n^r \frac{\log n}{\sqrt{n}} = k^r n^r \left(2^{-\Omega(r^2)} - \frac{2^{O(r^2)} k^r (\log n)}{\sqrt{n}}\right) \geq 0,$$
for $k$ as in the statement of the lemma for a sufficiently big constant $c$.  
\end{proof}

\subsection{Putting things together}\label{sec:wrapup}
We bring the arguments from previous sections together to prove our main results \tref{th:mainpsd} and \tref{th:main}.

\begin{proof}[Proof of \tref{th:mainpsd}]
Follows immediately from \lref{lm:subtofull} and \lref{lm:maintech}.
\end{proof}

\begin{proof}[Proof of \tref{th:main}] 
Follows immediately from \lref{lm:dualcert}, \clref{clm:dualsol} and \tref{th:mainpsd}.
\end{proof}

Theorems \ref{th:mainhierarchy} and \ref{cor:mainhierarchy} follow immediately from our $\psd$-refutation lower bound using standard arguments. We defer these to the appendix.

\input{technical}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> technical0305.tex <==
% !TEX root = main.tex

\section{Bounding norms of locally random matrices}\label{sec:localrand}
In this section we shall develop tools for bounding the norms of \emph{locally random} matrices (recall their informal definition from \sref{sec:outline} and more formal one in \sref{sec:normboundL}) associated with random graphs $G \lfta G(n,1/2)$, proving \clref{clm:maintechnicalL}. The idea behind our bounds is to use the \emph{trace method}. Recall the trace method: for any matrix $M$, for any positive integer $q$, $||M|| \leq \sqrt[2q]{tr(({M^T}M)^{q})}$ so we can probabilistically bound $||M||$ by bounding $\ex\sbkets{tr(({M^T}M)^{q})}$.

Going back to \clref{clm:maintechnicalL} let us first look at the special case of $a=1$ to gain some intuition. In this case, the entries of $R_1$ are (essentially) independent, and so the trace method is easy to apply. More precisely, $R_1$ is a symmetric random matrix with zeros on the diagonal and the entries in the upper diagonal taking independent uniformly random $\pm{1}$ values. It is well known that $\|R_1\| = O(\sqrt{n})$ in this case (see \cite{Vershynin06} for instance). One can also prove the bound by the trace method as follows. We have that  
$$\ex\sbkets{tr(({{R_1}^T}{R_1})^{q})} = \ex\sbkets{tr({R_1}^{2q})} = \sum_{i_1,\cdots,i_{2q}}{\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}},$$ where $i_{2q+1} = i_1$. We can then look at which products $\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}$ have expectation $0$. 

Since each individual ${R_1}({i_j},i_{j+1})$ is an independent $\pm{1}$ random variable with expectation $0$, a term in the summation $\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}} = 0$ unless every ${R_1}({i_j},i_{j+1})$ appears an even number of times in the product. Thus, the vast majority of the terms $\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}$ are $0$ and we can count the remaining terms to bound $\ex\sbkets{tr(R_1^{2q})}$.

\anote{Revised}

One way to visualize the above argument is to take terms $\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}$ and build a ``constraint graph'' for each term where the vertices correspond to the entries $\{i_j,i_{j+1}\}$, $j = 1,\ldots,2q$ appearing in the term. We then add edges between the vertices if the corresponding sets overlap (as a proxy for the dependence of the entries in $R$ - this happens here only if the same entry $(i,j)$, or its symmetric image $(j,i)$ appear in the term more than once). It is easy to argue now that any term with nonzero expected value must have a constraint graph with at most $q+1$ connected components. We can then bound the number of terms with nonzero expected value by the number of possible constraint graphs with at most $q+1$ connected components. This number can be bounded by $O((nq)^{q+1})$, so after picking the parameter $q$ optimally results in showing that with high probability  $\|R_1\| = O(\sqrt{n}\log n)$, a near-optimal bound.

To handle higher $a$'s we first generalize the above argument based on constraint graphs to work with general locally-random matrices. However, unlike for $a=1$, distinct entries of the matrix are now dependent, which significantly complicates the structure of constraint graphs and the associated count of the terms which are not zero. The rest of the section is devoted to this. While we apply our arguments to the particular locally-random matrices arising in our proof, these techniques should apply more generally to other locally-random matrices.  

%In this section we generalize these ideas to bound $||R_a||$ in two steps. In \sref{constraintgraphs} we develop tools for bounding the trace of high powers of locally random matrices. In \sref{rabounds} we apply these tools to the matrices $\{R_a\}$.
%--------------------------------------------------------------------------%
\subsection{Constraint graphs}\label{constraintgraphs}
%--------------------------------------------------------------------------%
We now formally introduce constraint graphs, which are a useful way to visualize terms in our calculations. We then prove a generic result bounding traces of high powers of locally random matrices (and some other functions) based on the structure of the associated constraint graphs; the advantage being that the conditions on the constraint graphs (in the form of bounds on the number of connected components) will be easier to ascertain in our applications. Here we use $V$ rather than $I$ for subsets because we will be viewing the individual elements of each $V$ as vertices.
\begin{definition}
Given a family of sets of vertices $\{V_i\}$, we define a corresponding constraint graph $C$ where
\begin{enumerate}
\item $V(C_{\{V_i\}}) = \{(V_i,j): j \in V_i\}$.
\item $E(C_{\{V_i\}}) = \{((V_{i_1},j),(V_{i_2},j)): j \in V_{i_1}, j \in V_{i_2}, V_{i_1} \neq V_{i_2}\}$.
\end{enumerate}
\end{definition}
\begin{theorem}\label{thm:productgraphtonorm}
Assume that we have values $\{s_1, \cdots, s_t\}$, a constant $B > 0$, and a function $p(G,2q)$ such that for every positive $q$, $p(G,2q) \geq 0$ and $p(G,2q)$ can be written in the form $p(G,2q) = \sum_{\{V_{ij}\}}{f(G,\{V_{ij}\})}$ where the following is true
\begin{enumerate}
\item $\{V_{ij}\}$ ranges over $i \in [1,q]$, $j \in [1,t]$, and subsets of vertices $V_{ij} \subseteq V(G)$
\item For all $i$ and $j$, $|V_{ij}| = s_j$
\item Taking $x = \sum_{j}{s_j}$ so that $qx$ is the total number of vertices in each constraint graph, for every term $f(G,\{V_{ij}\})$ with nonzero expected value, the corresponding constraint graph has at most $qx - qy + z$ connected components for some integers $y$ and $z$ where 
$1 \leq y \leq x$ and $z \geq 0$.
\item $\forall i,j, \ex[f(G,\{V_{ij}\})] \leq B^{2q}$
\end{enumerate}
then if $n \geq 10$, for all $\epsilon \in (0,1)$, 
$$\pr\left[|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}} \cdot \left(ex\Big(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\Big)\right)^y \cdot n^{\frac{x-y}{2}}\right] < \epsilon$$
\end{theorem}
\begin{remark}
We will use this theorem with two types of functions $p$. When $p(G,2q) = tr(({M^T}M)^q)$ for some matrix $M$ depending on $G$, 
$||M|| \leq \sqrt[2q]{p(G,2q)}$ for all $q > 0$ so this theorem gives us a probabilistic bound on $||M||$. When $p(G,2q) = h(G)^{2q}$ for some function $h$, then $h(G) = \sqrt[2q]{p(G,2q)}$ for all $q \in \mathbb{Z}^{+}$ so this theorem gives us a probabilistic bound on $h(G)$.
\end{remark}
\begin{example}
In the case when $p(G,2q) = tr(R_1^{2q})$, $p(G,2q) = \sum_{i_1,\cdots,i_{2q}}{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}$. Each term here has expected value at most $1$ and its corresponding constraint graph has 2q vertices. It can be shown 
(see \lref{lem:connectedcomponentbound}) that for any term with nonzero expected value, the constraint graph has at most $q+1$ connected components. Applying \tref{thm:productgraphtonorm} with $t = 2$, $\{s_1,s_2\} = \{1,1\}$, $V_{kl} = \{i_{2k+l-2}\}$, $x = 2$, $y = z = 1$, and $B = 1$ we have that if $n \geq 10$, for all $\epsilon \in (0,1)$, 
$$\pr\left[||R_1|| > 2e\sqrt{n} (\ln{n/\epsilon} + 2) \right] < \epsilon$$
This bound is a bit weaker than the bounds in e.g. \cite{Vershynin06}, but is sufficient for our purposes.
\end{example}
\begin{proof}[Proof of \tref{thm:productgraphtonorm}]
We prove this result by obtaining an upper bound on the number of terms in $p(G,2q) = \sum_{\{V_{ij}\}}{f(G,\{V_{ij}\})}$ with nonzero expected value. This gives us a probabilistic upper bound for $p(G,2q)$, implying the upper bound on $\min_q{\{\sqrt[2q]{p(G,2q)}\}}$.
\begin{definition}
Define $N(n,\{s_1,\cdots,s_t\},q,m)$ to be the number of ways to choose subsets $\{V_{ij}: i \in [1,2q], j \in [1,t]\}$ of $[n]$ such that $|\cup_{ij}{V_{ij}}| \leq m$ and for all $i,j$, $|V_{ij}| = s_j$.
\end{definition}
\begin{lemma}\label{tboundlemma}
Letting $x = 2\sum_{j}{s_j}$, if $m \leq qx$ then 
$$N(n,\{s_1,\cdots,s_t\},q,m) \leq \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}{\binom{qx}{qx-m}}{n^{m}}{{m}^{qx-m}}$$
\end{lemma}
\begin{proof}
We can choose each ordered $qx$-tuple $(v_1, \cdots, v_{qx})$ of elements in $[n]$ which contains at most $m$ distinct elements as follows. 
There must be at least $k-m$ elements which are duplicates of other elements, so we can first choose a set $I$ of $k-m$ indices such that for all $i \in I$, $v_i = v_j$ for some $j \notin I$. There are $\binom{qx}{qx-m}$ choices for $I$. We then choose the elements $\{v_j: j \notin I\}$. There are no restrictions on these elements so there are $n^{m}$ choices for these elements. Finally, we choose the elements $\{v_i: i \in I\}$. To determine each $v_i$ it is sufficient to specify the $j \notin I$ such that 
$v_i = v_j$. For each $i$ there are $m$ choices for the corresponding $j$, so the number of choices for these elements 
is at most $m^{qx-m}$. Putting everything together, the total number of choices is at most $\binom{qx}{qx-m}{n^{m}}{{m}^{qx-m}}$. Now note that since we are choosing subsets $\{V_{ij}: i \in [1,2q], j \in [1,t]\}$ of $[n]$ rather than one big ordered tuple, the order within each subset does not matter. Thus, there are $\left(\prod_{j=1}^{t}{{s_j}!}\right)^{2q}$ different ordered tuples which give the same subsets of elements, so the total number of possibilities for the subsets $\{V_{ij}\}$ is at most $\left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}{\binom{qx}{qx-m}}{n^{m}}{{m}^{qx-m}}$, as needed
\end{proof}
Now $E[p(G,2q)] = \sum_{\{V_{ij}\}}{E[f(G,\{V_{ij}\})]}$. For every nonzero term $E[f(G,\{V_{ij}\})]$ the corresponding constraint graph has at most $qx - qy + z$ connected components. If $q > \frac{z}{y}$ then applying \lref{tboundlemma} with $m = qx - qy + z$, there are at most 
\begin{align*}
\left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}\binom{qx}{qx-m}{n^{m}}{{m}^{qx-m}} &\leq 
\left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}{(qxm)}^{qx-m}{n^m} \\
&= \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}(qxm)^{yq}(qxm)^{-z}n^{(x-y)q}n^{z} \\
&= \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}(\frac{n}{qxm})^{z}\left((qxm)^{y}n^{x-y}\right)^{q} \\
&\leq \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}n^{z}\left((q^2x^2)^{y}n^{x-y}\right)^{q}
\end{align*}
nonzero terms $E[f(G,\{V_{ij}\})]$
Moreover, by our assumptions, each of these nonzero terms $E[f(G,\{V_{ij}\})]$ has value at most $B^{2q}$, so $$E[p(G,2q)] \leq \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}n^{z}\left((q^2x^2)^{y}n^{x-y}\right)^{q}B^{2q}$$
Thus, for all $q > \frac{z}{y}$, 
$$E[p(G,2q)] \leq n^{z}\left(B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}}(qx)^{y}n^{\frac{x-y}{2}}\right)^{2q}$$
Using Markov's inequality, 
$$\epsilon > P\left(|p(G,2q)| > \frac{1}{\epsilon}E[p(G,2q)]\right) \geq P\left(|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > 
\sqrt[2q]{\frac{1}{\epsilon}E[p(G,2q)]}\right)$$
Combining these two equations gives
$$P\left(|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > \frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}}
(B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}}x^{y}n^{\frac{x-y}{2}})\right) < \epsilon$$
We will try to minimize $\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}}$ with respect to $q$. 
Setting the derivative to $0$ gives 
$$\left(\frac{y}{q} - \frac{z\ln{n} - \ln{\epsilon}}{2q^2}\right)
\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}} = 0$$
This occurs when $q = \frac{z\ln{n} - \ln{\epsilon}}{2y}$. We need $q$ to be an integer so we set $q$ to be the smallest 
integer which is at least $\frac{z\ln{n} - \ln{\epsilon}}{2y}$. As long as $n \geq 10$ this guarantees that $q > \frac{z}{y}$. 
Now $q < \frac{z\ln{n} - \ln{\epsilon}}{2y} + 1$ and 
$$\left(\frac{n^z}{\epsilon}\right)^{\frac{1}{2q}} \leq 
\left(e^{z\ln{n} - \ln{\epsilon}}\right)^{\frac{y}{z\ln{n} - \ln{\epsilon}}} = e^y$$
Thus, for this $q$, 
$$\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}} \leq e^y\left(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\right)^y$$
Putting everything together, 
$$P\left(|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > e^y\left(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\right)^y
(B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}}x^{y}n^{\frac{x-y}{2}})\right) < \epsilon$$
and rearranging gives the desired result.
\end{proof}
%--------------------------------------------------------------------------%
\subsection{Bounds on $||R_a||$}\label{rabounds}
%--------------------------------------------------------------------------%
In this subsection, we prove \clref{clm:maintechnicalL} using \tref{thm:productgraphtonorm}. For convenience, we restate \clref{clm:maintechnicalL} here with more precise constants.
\begin{theorem}\label{th:rabounds}
If $n \geq 100$, for all $\epsilon \in (0,1)$, 
$\pr\left[||R_a|| > 2^{a^2+2a+2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon$.
\end{theorem}

We prove the theorem by applying \tref{thm:productgraphtonorm}. The core of the argument will be to bound the number of connected components in the constraint graphs of terms $\prod_{j=1}^{2q} R_a(V_{i_j}, V_{i_{j+1}})$ with non-zero expectation which appear in the expansion of $tr((R_a^T R_a)^q)$. We will show that the number of connected components is at most $2aq - q + 1$ (note that $2aq$ is a trivial bound as the number of vertices in the constraint graph is $4aq$ and no vertex can be isolated in a non-zero term). We will prove this bound by inductively decomposing $R_a$ as follows. 
%To make the proof cleaner, we further decompose $R_a$ as follows.
\begin{definition}
Given a partition $(A,B)$ of $[1,n]$, define $R_{a,A,B}(V_1,V_2) = R_{a}(V_1,V_2)$ if $V_1 \subseteq A$ and $V_2 \subseteq B$ and $0$ otherwise.
\end{definition}
\begin{proposition}
$\sum_{A,B}{R_{a,A,B}} = 2^{n-2a}R_a$
\end{proposition}
\begin{proof}
$R_{a,A,B}(V_1,V_2) = R_a(V_1,V_2) = 0$ whenever $V_1$ and $V_2$ are not disjoint. For all disjoint $V_1$ and $V_2$, $R_{a,A,B}(V_1,V_2) = R_a(V_1,V_2)$ for $2^{n-2a}$ choices of $A$ and $B$ and is $0$ for the rest.
\end{proof}
\begin{corollary}\label{cor:parttowhole}
$||R_a|| \leq 2^{2a}\max_{A,B}{\{||R_{a,A,B}||\}}$
\end{corollary}
\begin{proof}
Since $R_a = 2^{2a-n}\sum_{A,B}{R_{a,A,B}}$, $||R_a|| \leq 2^{2a-n}\sum_{A,B}{||R_{a,A,B}||} \leq 2^{2a}\max_{A,B}{\{||R_{a,A,B}||\}}$
\end{proof}
Now given $A$ and $B$, take 
\begin{align*}
p(G,2q) = tr((R^T_{a,A,B}R_{a,A,B})^q) &= \sum_{\{V_{ij}: i \in [1,q], j \in [1,2]\}}{\prod_{i=1}^{q}{R^T_{a,A,B}(V_{i1},V_{i2})R_{a,A,B}(V_{i2},V_{(i+1)1})}} \\
&= \sum_{{\{V_{ij}: i \in [1,q], j \in [1,2]\}: \atop \forall i, V_{i1} \subseteq B} \atop {\forall i, V_{i2} \subseteq A}}
{\prod_{i=1}^{q}{R_{a}(V_{i1},V_{i2})R_{a}(V_{i2},V_{(i+1)1})}}
\end{align*} 
where we take $V_{(q+1)1} = V_{11}$. 

To simplify this expression, rename the sets of vertices as follows.
\begin{definition} \ 
\begin{enumerate}
\item If $i \in [1,2q]$ and $i$ is odd then take $W_i = V_{(\frac{i+1}{2})1}$
\item If $i \in [1,2q]$ and $i$ is even then take $W_i = V_{(\frac{i}{2})2}$
\end{enumerate}
\end{definition}
We now have that 
$$p(G,2q) = \sum_{{{\{W_i}: i \in [1,2q]\}: \atop \forall \text{ odd } i, W_{i} \subseteq B} \atop {\forall \text { even } i, W_{i} \subseteq A}}{\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}}$$
where we take $W_{2q + 1} = W_1$. Now let's consider which of these terms have expectation $0$. Each $R_{a}(W_{i},W_{i+1})$ is a random variable with expectation $0$, so if any $R_{a}(W_{i},W_{i+1})$ is independent from everything else, the product will have expectation $0$. Each $R_{a}(W_{i},W_{i+1})$ is independent from everything else precisely when none of the edges between $W_{i}$ and $W_{i+1}$ appear anywhere else. Thus, we only need to count the terms such that for all $i$ there is a $j \neq i$ such that some edge between $W_{i}$ and $W_{i+1}$ is also an edge between $W_{j}$ and $W_{j+1}$.

We express this condition in terms of the constraint graphs as follows. We first define a related graph $H$ which is easier to work with and analyze.
\begin{definition}
Given a constraint graph $G$, let $H$ a graph with two types of edges, product edges and constraint edges, such that 
\begin{enumerate}
\item $V(H) = \{W_i: i \in [1,2q]\}$
\item $E_{product}(H) = \{(W_i,W_{i+1}): i \in [1,2q]\}$
\item $E_{constraint}(H) = \{(W_i,W_j): i \neq j, W_i \cap W_j \neq \emptyset\}$
\end{enumerate}
\end{definition}
We now define the concept of an independence breaking cycle on $H$ so that for each $i$, 
there is a $j \neq i$ such that some edge is both between $W_i$ and $W_{i+1}$ and between $W_j$ and $W_{j+1}$ if and only if the product edge $(W_{i},W_{i+1})$ is part of an independence-breaking cycle. This implies each product $\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}$ has zero expected value unless all of the product edges in the corresponding $H$ are part of independence-breaking cycles. This places restrictions on $H$ (see \lref{lem:connectedcomponentbound}) which in turn places restrictions on the constraint graph $C$, allowing us to use \tref{thm:productgraphtonorm}. We make these ideas precise below.
\begin{definition}
Given $q$ and $\{W_1, \cdots, W_{2q}\}$, we define $W_{i \pm 2q} = W_{i}$ for all $i \in [1,2q]$.
\end{definition}
\begin{definition} If $q \geq 2$, 
\begin{enumerate}
\item Define an independence breaking 3-cycle in $H$ to consist of product edges $(W_i,W_{i+1})$, $(W_{i+1},W_{i+2})$ 
and a constraint edge $((W_{i},j),(W_{i+2},j))$.
\item Define an independence breaking 4-cycle to consist of product edges $e_1 = (W_{i_1},W_{i_1+1})$, 
$e_2 = (W_{i_2},W_{i_2 \pm 1})$ and constraint edges $(W_{i_1},W_{i_2})$ and $(W_{i_1 + 1},W_{i_2 \pm 1})$.
\end{enumerate}
\end{definition}
\begin{proposition}
For all $W_1, \cdots, W_{2q}$ such that $W_i \subseteq B$ whenever $i$ is odd and $W_i \subseteq A$ whenever $i$ is even, if the corresponding $H$ has a product edge $(W_i,W_{i+1})$ which is not contained in any independence-breaking cycle then $E[\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}] = 0$
\end{proposition}
\begin{proof}
If $(W_i,W_{i+1})$ is not contained in any independence-breaking cycle then no edge between $W_i$ and $W_{i+1}$ appears anywhere else so $R_{a}(W_{i},W_{i+1})$ is a random variable with expectation $0$ which is independent from everything else and thus $E[\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}] = 0$.
\end{proof}
We now bound the number of connected components in $H$ with the following lemma.
\begin{lemma}\label{lem:connectedcomponentbound}
If $q \geq 2$ and $H$ is a graph such that
\begin{enumerate}
\item Every product edge of $H$ is contained in an independence-breaking cycle.
\item Every constraint edge of $H$ is of the form $(W_i,W_{i+j})$ where $j$ is even.
\end{enumerate} 
then looking only at the constraint edges, the number of connected components of $H$ is at most $q+1$.
\end{lemma}
The intuitive idea behind this lemma is that if we add the constraint edges in the right order, every new constraint edge can put two product edges into independence breaking cycles. For example, a constraint edge between $W_{i-1}$ and $W_{i+1}$ puts the product edges $(W_{i-1},W_i)$ and $(W_i,W_{i+1})$ into an independence breaking 3-cycle. If we then add a constraint edge between $W_{i-2}$ and $W_{i+2}$, this puts the product edges $(W_{i-2},W_{i-1})$ and $(W_{i+1},W_{i+2})$ into an independence breaking 4-cycle. The final constraint edge can put 4 product edges into independence breaking cycles, so the number of constraint edges needed is $q-1$.

to make this argument work, we use an inductive proof. We note that if there is no $W_i$ which is isolated in $H$, we must have at least $q$ constraint edges. On the other hand, if there a $W_i$ which is isolated, there must be a constraint edge between $W_{i-1}$ and $W_{i+1}$. As noted above, this constraint edge puts the product edges $(W_{i-1},W_i)$ and $(W_i,W_{i+1})$ into an independence breaking 3-cycle. We take this to be the first constraint edge. We then argue that we can essentially delete $W_i$ and merge $W_{i-1}$ and $W_{i+1}$ which allows us to use the inductive hypothesis. We make these ideas rigorous below.
\begin{proof}[Proof of \lref{lem:connectedcomponentbound}]
We prove \lref{lem:connectedcomponentbound} by induction on $q$. The base case $q = 2$ is trivial, as we clearly need at least one constraint edge, so the number of connected components in $H$ is at most $3$. 
Now assume that $q = k \geq 3$ and the result is true for $q = k-1$.

First note that if there is no $W_i$ which is isolated, then there are at most 
$q$ connected components in $H$. Thus, we may assume that $W_i$ is isolated for some $i$. Now 
note that for the product edge $(W_{i-1},W_{i})$, since $W_i$ is isolated, there are no independence breaking 3-cycles or 4-cycles where $W_i$ is the endpoint of a constraint edge. 
Thus, we must have that $(W_{i-1},W_{i})$ is part of an independence breaking 3-cycle consisting of $(W_{i-1},W_i)$, $(W_i,W_{i+1})$, and 
a constraint edge $(W_{i-1},W_{i+1})$.

Now form a new graph $H'$ as follows. Delete $W_i$ and contract the constraint edge between $W_{i-1}$ and $W_{i+1}$. More precisely, 
\begin{enumerate}
\item Take $V(H') = V(H) \setminus \{W_{i-1},W_i,W_{i+1}\} \cup \{U\}$
\item Take $E_{product}(H') = E_{product}(H) \setminus \{(W_{i},W_{i+1}): i \in [i-2,i+1]\} \cup \{(W_{i-2},U),(U,W_{i+2})\}$
\item Take \begin{align*}
E_{constraint}(H') &= E_{constraint}(H) \setminus \{(W_{i-1},W_{j}): (W_{i-1},W_{j}) \in E_{constraint}(H)\} \\
&\setminus \{(W_{i+1},W_{j}): (W_{i+1},W_{j}) \in E_{constraint}(H)\} \\
&\cup \{(U,W_{j}): (W_{i-1},W_{j}) \in E_{constraint}(H) \text{ or } (W_{i+1},W_{j}) \in E_{constraint}(H)\}
\end{align*}
\end{enumerate}
After doing this, rename $U$ as $W_{i-1}$ and rename each $W_{j}$ where $j > i+1$ as $W_{j-2}$. In going from $H$ to $H'$, we have effectively reduced both $q$ and the number of connected components by $1$. To complete the proof, we need to check that $H'$ satisfies the inductive hypotheses. Based on the reduction from $H$ to $H'$, we still have that every constraint edge is of the form $(W_i,W_{i+j})$ where $j$ is even. We check that every product edge is still part of an independence-breaking cycle case by case. 
\begin{enumerate}
\item Every independence-breaking cycle which did not contain the constraint edge $(W_{i-1},W_{i+1})$ in $H$ is preserved in $H'$ except that the vertices may have been renamed. The reason for this is that such an independence breaking cycle in $H$ cannot contain $W_i$ and can contain at most one of $\{W_{i-1},W_{i+1}\}$.
\item The independence-breaking 3-cycle in $H$ consisting of the product edges $(W_{i-1},W_{i})$, $(W_{i},W_{i+1})$ and the constraint edge $(W_{i-1},W_{i+1})$ is removed, but so are the product edges $(W_{i-1},W_{i})$ and $(W_{i},W_{i+1})$, so this is fine.
\item If we have an independence breaking 4-cycle in $H$ consisting of the product edges $(W_{i-2},W_{i-1})$, $(W_{i+1},W_{i+2})$ and the constraint edges $(W_{i-1},W_{i+1})$, $(W_{i-2},W_{i+2})$, this becomes an independence-breaking 3-cycle in $H'$ with product edges $(W_{i-2},W_{i-1})$, $(W_{i-1},W_{i})$ and a constraint edge $(W_{i-2},W_{i})$ (note that $W_{i-1}$ and $W_{i+1}$ are merged into $W_{i-1}$ in $H'$ and $W_{i+2}$ is renamed as $W_i$ in $H'$).
\end{enumerate}
$H'$ satisfies the inductive hypotheses, so looking only at the constraint edges, $H'$ has at most $(q-1)+1 = q$ connected components. $H$ has one more connected component than $H'$ (the vertex $W_i$ in $H$), so $H$ has at most $q+1$ connected components, as needed.
\end{proof}
\begin{remark}
The fact that $W_i \subseteq B$ whenever $i$ is odd and $W_i \subseteq A$ is even saved us from considering the possibility that we had an independence breaking 4-cycles consisting of product edges $(W_{i+1},W_{i+2})$, $(W_{i-2},W_{i-1})$ and constraint edges $(W_{i-1},W_{i+2})$, $(W_{i-2},W_{i+1})$. Such an independence-breaking 4-cycle would be contracted into a 4-cycle with only three vertices. We could have modified the definition of independence-breaking 4-cylces to include this possibility, but it is cleaner and easier to think about when we avoid this case and other weird cases entirely. 
\end{remark}
We now use this bound on the number of connected components of $H$ to prove a corresponding bound on the number of connected components of $C$.
\begin{proposition}
For all constraint graphs $C$ and the corresponding graphs $H$, $|V(C)|$ minus the number of connected components of $C$ is at least as large as $|V(H)|$ minus the number of connected components of $H$.
\end{proposition}
\begin{proof}
Consider the process of starting with $V(H)$ and then adding edges of $H$ one at a time where each new edge reduces the number of connected components until this is no longer possible. The number of edges we add is $|V(H)|$ minus the number of connected components of $H$. Now note that if we start with $V(C)$ and add the corresponding edges in $C$, this already reduces the number of connected components by the number of edges we added and the result follows.
\end{proof}
\begin{corollary}
For all terms with nonzero expectation, $C$ has at most $2aq - q + 1$ connected components
\end{corollary}
We can now prove \tref{th:rabounds}
\begin{proof}[Proof of \tref{th:rabounds}]
We can now apply \tref{thm:productgraphtonorm} with $t=2$, $s_1 = s_2 = a$, $x = 2a$, $y = 1$, and $z = 1$. Every entry of $R_{a,A,B}$ has magnitude at most $2^{a^2}$ so we can take $B = 2^{a^2}$. By \tref{thm:productgraphtonorm}, if $n \geq 10$, for all $A$ and $B$, for every $\epsilon \in (0,1)$, 
$$\pr\left[||R_{a,A,B}|| > \frac{2^{a^2}}{a!}\left(2ea\Big(\frac{\ln{n} - \ln{\epsilon}}{2} + 1\Big)\right)
n^{\frac{2a-1}{2}}\right] = 
\pr\left[||R_{a,A,B}|| > \frac{2^{a^2}ea}{a!}(\ln{n} - \ln{\epsilon} + 2)
n^{a - \frac{1}{2}}\right] < \epsilon$$
Since $4\ln{n} \geq e(\ln{n} + 2)$ for all $n \geq 100$ and $a! \geq a$, we have that for all $n \geq 100$, for all $A$ and $B$ and all $\epsilon \in (0,1)$, 
$$\pr\left[||R_{a,A,B}|| > 2^{a^2+2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon$$
Now by \cref{cor:parttowhole}, $||R_a|| \leq 2^{2a}\max_{A,B}{\{||R_{a,A,B}||\}}$ so $$\pr\left[||R_{a}|| > 2^{a^2 + 2a + 2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon$$
\end{proof}

%%% Local Variables:   
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> technical20305.tex <==
% !TEX root = main.tex

%--------------------------------------------------------------------------%
\section{Concentration bounds for number of cliques and $deg_G(I)$}\label{sec:degreevariancecalculations}
%--------------------------------------------------------------------------%
\begin{definition}
For a graph $G$, define $N_a(G)$ to be the number of $a$-cliques in $G$.
\end{definition}
In this section, we prove the following large-deviation bounds on $N_a(G)$ and on $deg_G(I)$ for small sets of vertices $I$:
\begin{theorem}\label{cliqueboundtheoremone}
For all $a$, for all $n \geq 10$ and $\epsilon \in (0,1)$, $E[N_a(G)] = 2^{-\binom{a}{2}}{\binom{n}{a}}$ and 
$$\pr\left[|N_a(G) - E[N_a(G)]| > (\ln(\frac{64}{\epsilon}))^2 \cdot n^{a-1}\right] < \epsilon$$
\end{theorem}
\begin{definition}
Given any $I \subseteq [n]$, let $A_I$ be the set of all vertices not in $I$ which are adjacent to all 
vertices in $I$.
\end{definition}
\begin{theorem}\label{cliqueboundtheoremtwo}
If $n \geq 10$ and $\epsilon \in [6e^{-\frac{n-2r}{2^{2r} \cdot 2r \cdot \sqrt{n}}},1]$ then
$$P\left[\left|deg_G(I) - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|} - 
2^{\binom{|I|}{2}-\binom{2r}{2} + |I|}\frac{(n-|I|)^{2r-|I|-1}}{(2r-|I|-1)!}\Delta_{I}\right| > 20(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1}\right] < \epsilon$$
Less precsiely, 
$$P\left[\left|deg_G(I) - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|}\right| > 8(\ln(\frac{6}{\epsilon}))n^{2r-|I|-\frac{1}{2}}\right] < \epsilon$$
\end{theorem}
%--------------------------------------------------------------------------%
\subsection{Concentration bounds for $N_a(G)$}
%--------------------------------------------------------------------------%
We first prove concentration bounds for $N_a(G)$ because these bounds are easier and are the basis for the concentration bounds on $deg_G(I)$. While similar results appear in the literature, see for instance \cite{Rucinski88, Vu01, JLR11book}, we give a short direct proof here to obtain explicit constants.\\
{\bf Theorem \ref{cliqueboundtheoremtwo}.}
{\it
For all $a$, for all $n \geq 10$ and $\epsilon \in (0,1)$, $E[N_a(G)] = 2^{-\binom{a}{2}}{\binom{n}{a}}$ and 
$$\pr\left[|N_a(G) - E[N_a(G)]| > (\ln(\frac{64}{\epsilon}))^2 \cdot n^{a-1}\right] < \epsilon$$
}
\begin{proof}
The first part of the theorem is trivial so we focus on the second part.
\begin{definition}
Given a set of vertices $V$ of size $a$, define $c_V$ to be $1-2^{-\binom{a}{2}}$ if $V$ is a clique and $-2^{-\binom{a}{2}}$ otherwise
\end{definition}
\begin{proposition}
$N_a(G) - E[N_a(G)] = \sum_{V:|V| = a}{c_V}$
\end{proposition}
Now let's consider the function 
$p(G,2q) = (\sum_{V:|V| = a}{c_V})^{2q} =\sum_{W_1, \cdots, W_{2q}}{\prod_{i=1}^{2q}{c_{W_i}}}$

Note that $E[\prod_{i=1}^{2q}{c_{W_i}}] = 0$ unless each set of vertices $W_i$ has two vertices in common with a different set of vertices $W_j$. This implies that when we look at the constraint graphs for the terms with nonzero expected value, for every $i$, the set of vertices $\{(W_i,v): v \in W_i\}$ is incident with at least two constraint edges. Note that the total number of vertices in each constraint graph is $2qa$ so this in turn implies that each such constraint graph has at most $2qa - 2q$ connected components.

Taking $V_{ij}=W_{2i+j-2}$ for $i \in [1,q]$ and $j \in [1,2]$, we can now apply \tref{thm:productgraphtonorm} with $s_1 = s_2 = a$, $x=2a$, $y=2$, $z=0$, and $B = 1$. Using \tref{thm:productgraphtonorm}, if $n \geq 10$, for all $\epsilon \in (0,1)$, 
$$\pr\left[|N_a(G) - E[N_a(G)]| > \frac{1}{a!} \cdot \left(ea\Big(\frac{-\ln{\epsilon}}{4} + 1\Big)\right)^2 \cdot n^{a-1}\right] < \epsilon$$
Using the facts that $e^2 < 8$ and $\frac{m^2}{m!} \leq 2$ for all nonnegative integers $m$, we have that 
$$\pr\left[|N_a(G) - E[N_a(G)]| > (\ln(\frac{64}{\epsilon}))^2 \cdot n^{a-1}\right] < \epsilon$$
\end{proof}
%--------------------------------------------------------------------------%
\subsection{Concentration bounds for $deg_G(I)$}
%--------------------------------------------------------------------------%
Now that we have proven \tref{cliqueboundtheoremone}, we will derive \tref{cliqueboundtheoremtwo} 
from \tref{cliqueboundtheoremone}. The idea is that conditioned on $I$ being a clique, by 
Theorem \tref{cliqueboundtheoremone}, $deg_G(I)$ is primarily determined by $|A_I|$, which can be easily shown to be tightly concentrated around its expected value. We make this argument rigorous below.
\vskip.1in
\noindent
{\bf Theorem \ref{cliqueboundtheoremtwo}.}
{\it
If $n \geq 10$ and $\epsilon \in [6e^{-\frac{n-2r}{2^{2r} \cdot 2r \cdot \sqrt{n}}},1]$ then
$$P\left[\left|deg_G(I) - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|} - 
2^{\binom{|I|}{2}-\binom{2r}{2} + |I|}\frac{(n-|I|)^{2r-|I|-1}}{(2r-|I|-1)!}\Delta_{I}\right| > 20(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1}\right] < \epsilon$$
Less precsiely, 
$$P\left[\left|deg_G(I) - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|}\right| > 8(\ln(\frac{6}{\epsilon}))n^{2r-|I|-\frac{1}{2}}\right] < \epsilon$$
}
\begin{proof}[Proof of \tref{cliqueboundtheoremtwo}]
The result is trivial if $|I| = 2r$ and follows immediately from Theorem \ref{cliqueboundtheoremone} if $|I| = 0$ 
so we may assume that $0 < |I| < 2r$. We first prove elementary concentration bounds on $|A_I|$. We then analyze $deg_G(I)$ assuming that these bounds hold.
\begin{definition}
for all $a$, define $E_a = 2^{-a}(n-|a|)$
\end{definition}
\begin{definition}
For any $I \subseteq V(G)$, define $\Delta_I = |A_I| - E_{|I|}$
\end{definition}
\begin{proposition}
For all $I$, $|A_I| = E_{|I|} + \Delta_I$.
\end{proposition}
\begin{lemma}\label{avboundslemma}
If $n \geq 10$, for all $\epsilon \in (0,1)$, $\pr\left[|\Delta_I| > 2\ln{(\frac{6}{\epsilon})}\sqrt{n}\right] < \frac{\epsilon}{2}$
\end{lemma}
\begin{proof}
Consider the function $p(G,2q) = (\Delta_I)^{2q} = \sum_{v_1,\cdots,v_2q}{\prod_{l=1}^{2q}{a(I,v_l)}}$ where $a(I,v)$ is $0$ if $v \in I$, $a(I,v) = 1-2^{-|I|}$ if $v \notin I$ and there is an edge between $v$ and every element of $I$ in $G$, and $a(I,v) = -2^{-|I|}$ otherwise.

All constraint graphs have $2q$ vertices. Note that $\prod_{j=1}^{2q}{a(I,v_j)}$ has zero expectation unless each $v_{j}$ is duplicated, so for any term with nonzero expected value, there are at most $q$ connected components. Taking $V_{ij}= \{v_{2i+j-2}\}$ for $i \in [1,q]$ and $j \in [1,2]$, we can now apply \tref{thm:productgraphtonorm} with $s_1 = s_2 = 1$, $x=2$, $y=1$, $z=0$, and $B = 1$. Using \tref{thm:productgraphtonorm}, if $n \geq 10$, for all $\epsilon_2 \in (0,1)$, 
$$\pr\left[|\Delta_I| > e(\frac{-\ln{(\epsilon_2)}}{2} + 1)\sqrt{n}\right] < \epsilon_2$$
Applying this with $\epsilon_2 = \frac{\epsilon}{2}$ and simplifying, we have that
$$\pr\left[|\Delta_I| > 2\ln{(\frac{6}{\epsilon})}\sqrt{n}\right] < \frac{\epsilon}{2}$$
\end{proof}
Now note that $deg_G(I)$ is equal to the number of cliques of size $2r-|I|$ in $A_I$. Applying \tref{cliqueboundtheoremone} 
with $\frac{\epsilon}{2}$, if $n \geq 10$, 
\begin{equation}\label{deggiequation}
\pr\left[\left|deg_G(I) - 2^{-\binom{2r - |I|}{2}}\binom{|A_I|}{2r - |I|}\right| > (\ln(\frac{128}{\epsilon}))^2 \cdot |A_I|^{2r-|I|-1}\right] < \frac{\epsilon}{2}
\end{equation} 
We now estimate $\binom{|A_I|}{2r - |I|}$ assuming that $|\Delta_I| \leq 2\ln{(\frac{6}{\epsilon})}\sqrt{n}$
\begin{lemma}\label{approximationslemma}
If $0 < |I| < 2r$, $|\Delta_I| \leq 2\ln{(\frac{6}{\epsilon})}\sqrt{n}$, and $|\Delta_I| \leq \frac{E_{|I|}}{(2r-|I|)}$ then 
$$\left|\binom{|A_I|}{2r - |I|} - 2^{-|I|(2r-|I|)}\binom{n-|I|}{2r - |I|} - 
\frac{(2r - |I|)\Delta_{I}(E_{|I|})^{2r-|I|-1}}{(2r-|I|)!}\right| \leq 10(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1}$$
\end{lemma}
\begin{proof}
We split this expression into three parts
\begin{enumerate}
\item $\binom{|A_I|}{2r - |I|} - \frac{|A_I|^{2r-|I|}}{(2r - |I|)!}$
\item $\frac{|A_I|^{2r-|I|}}{(2r - |I|)!} - \frac{(E_{|I|})^{2r-|I|}}{(2r - |I|)!} - 
\frac{(2r-|I|)\Delta_{I}(E_{|I|})^{2r-|I|-1}}{(2r - |I|)!}$
\item $\frac{(E_{|I|})^{2r-|I|}}{(2r - |I|)!} - 2^{-|I|(2r-|I|)}\binom{n-|I|}{2r - |I|}$
\end{enumerate}
For the first and third parts, we can use the following proposition.
\begin{proposition}\label{factorialapproxprop}
For all nonnegative integers $m$ and $k$ where $k < m$, $0 \leq \frac{m^k}{k!} - {m \choose k} \leq \frac{k^2}{2}\frac{m^{k-1}}{k!}$
\end{proposition}
\begin{proof}
Note that $m^k \geq \prod_{j=0}^{k-1}{(m-j)} \geq m^k\prod_{j=0}^{k-1}{(1 - \frac{j}{m})} \geq 
m^k(1 - \sum_{j=0}^{k-1}{\frac{j}{m}}) \geq m^k(1 - \frac{k^2}{2m})$

This implies that $0 \leq m^k - \prod_{j=0}^{k-1}{(m-j)} \leq \frac{k^2}{2m}{m^k}$ and dividing everything by 
$k!$ gives the claimed result.
\end{proof}
Using Proposition \ref{factorialapproxprop} with $k = 2r-|I|$ and $m = |A_I|$, $m = n-|I|$ respectively,
\begin{enumerate}
\item $\left|\binom{|A_I|}{2r - |I|} - \frac{|A_I|^{2r-|I|}}{(2r - |I|)!}\right| 
\leq \frac{(2r-|I|)^2}{2}\frac{|A_I|^{2r-|I|-1}}{(2r-|I|)!} \leq n^{2r-|I|-1}$
\item 
\begin{align*}
\left|\frac{(E_{|I|})^{2r-|I|}}{(2r - |I|)!} - 
2^{-|I|(2r-|I|)}\binom{n-|I|}{2r - |I|}\right| &= \left|2^{-|I|(2r-|I|)}\frac{(n-|I|)^{2r-|I|}}{(2r - |I|)!} - 
2^{-|I|(2r-|I|)}\binom{n-|I|}{2r - |I|}\right| \\
&\leq 2^{-|I|(2r-|I|)}\frac{(2r-|I|)^2}{2}\frac{(n-|I|)^{2r-|I|-1}}{(2r-|I|)!} \\
&\leq \frac{n^{2r-|I|-1}}{2}
\end{align*}
\end{enumerate}
For the second part, note that the result is trivial when $|I| = 2r-1$ so we may assume that $0 < |I| < 2r-1$. We can now use the following proposition.
\begin{proposition}\label{linearapproximationprop}
For any nonnegative integer $k$ and any $x$ such that $|kx| \leq 1$, $\left|(1+x)^k - (1 + kx)\right| \leq {k^2}{x^2}$
\end{proposition}
\begin{proof}
$$\left|(1+x)^k - (1 + kx)\right| \leq \sum_{j=2}^{k}{\left|{k \choose j}{x^j}\right|} 
\leq \sum_{j=2}^{k}{\left|\frac{1}{j!}{k^j}{x^j}\right|} \leq {k^2}{x^2}\sum_{j=2}^{k}{\frac{1}{j!}} \leq {k^2}{x^2}$$
\end{proof}
Using Proposition \ref{linearapproximationprop} with $k=2r-|I|$ and $x = \frac{\Delta_I}{E_{|I|}}$, if 
$|\Delta_I| \leq \frac{E_{|I|}}{(2r-|I|)}$
\begin{align*}
&\left|\frac{|A_I|^{2r-|I|}}{(2r - |I|)!} - 
\frac{(E_{|I|})^{2r-|I|}}{(2r - |I|)!} - 
\frac{(2r-|I|)\Delta_{I}(E_{|I|})^{2r-|I|-1}}{(2r - |I|)!}\right| = \\
&\frac{(E_{|I|})^{2r-|I|}}{(2r - |I|)!}\left|(1+\frac{\Delta_I}{E_{|I|}})^{2r - |I|} - 
1 - (2r-|I|)\frac{\Delta_I}{E_{|I|}}\right| \\
& \leq \frac{(E_{|I|})^{2r-|I|}}{(2r - |I|)!}\frac{(2r-|I|)^2(\Delta_I)^2}{(E_{|I|})^2} \\
& \leq 2(E_{|I|})^{2r-|I|-2}(\Delta_I)^2 \leq 2n^{2r-|I|-2}(\Delta_I)^2
\end{align*}
Since $|\Delta_I| \leq 2\ln{(\frac{6}{\epsilon})}\sqrt{n}$, this is at most $8(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1}$. The result now follows from adding these three parts together.
\end{proof}
\begin{corollary}\label{approximationscorollary}
For all $n \geq 10$, for all $\epsilon \in (0,1)$, if $0 < |I| < 2r$ and 
$|\Delta_I| \leq 2\ln{(\frac{6}{\epsilon})}\sqrt{n} \leq \frac{E_{|I|}}{(2r-|I|)}$ then 
$$\left|\binom{|A_I|}{2r - |I|} - 2^{-|I|(2r-|I|)}\binom{n-|I|}{2r - |I|}\right| 
\leq 5(\ln(\frac{6}{\epsilon}))n^{2r-|I|-\frac{1}{2}}$$
\end{corollary}
\begin{proof}
\lref{approximationslemma} says that 
$$\left|\binom{|A_I|}{2r - |I|} - 2^{-|I|(2r-|I|)}\binom{n-|I|}{2r - |I|} - 
\frac{(2r - |I|)\Delta_{I}(E_{|I|})^{2r-|I|-1}}{(2r-|I|)!}\right| \leq 10(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1}$$
Since $|\Delta_I| \leq 2\ln{(\frac{6}{\epsilon})}\sqrt{n}$ and $E_{|I|} \leq n$ we have that 
$\left|\frac{(2r - |I|)\Delta_{I}(E_{|I|})^{2r-|I|-1}}{(2r-|I|)!}\right| < 2\ln{(\frac{6}{\epsilon})}n^{2r-|I|-\frac{1}{2}}$ 

Since $2\ln{(\frac{6}{\epsilon})}\sqrt{n} \leq \frac{E_{|I|}}{(2r-|I|)}$ and $E_{|I|} \leq \frac{n}{2}$, 
$$10(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1} \leq 5\ln{(\frac{6}{\epsilon})}\frac{E_{|I|}}{2r-|I|}n^{2r-|I|-\frac{3}{2}} < 3\ln{(\frac{6}{\epsilon})}n^{2r-|I|-\frac{1}{2}}$$
Combining these equations gives the result.
\end{proof}
We now put everything together to prove \ref{cliqueboundtheoremtwo}. The condition that 
$\epsilon \geq 6e^{-\frac{n-2r}{2^{2r} \cdot 2r \cdot \sqrt{n}}}$ ensures that $2\ln{(\frac{6}{\epsilon})}\sqrt{n} \leq \frac{E_{|I|}}{(2r-|I|)}$ whenever $0 < |I| < 2r$ so we may apply \lref{approximationslemma} and Corollary \ref{approximationscorollary} whenever $|\Delta_I| \leq 2\ln{(\frac{6}{\epsilon})}\sqrt{n}$, which by \lref{avboundslemma} happens with probability at least 
$1-\frac{\epsilon}{2}$. We now make the following observation
\begin{proposition}\label{rephrasingprop}
$2^{-\binom{2r - |I|}{2}} \cdot 2^{-|I|(2r-|I|)} = 2^{\binom{|I|}{2}-\binom{2r}{2}}$
\end{proposition}
\begin{proof}
This follows from the equation $\binom{2r}{2} = \binom{2r - |I|}{2} + |I|(2r-|I|) + \binom{|I|}{2}$ which just says that to pick two elements from $[1,2r]$ we ca either pick two elements from $[1,2r-|I|]$, pick one element from $[1,2r-|I|]$ and one element from $[2r-|I|+1,2r]$, or pick two elements from $[2r-|I|+1,2r]$.
\end{proof}
Using Proposition \ref{rephrasingprop}, 
\begin{enumerate}
\item $2^{-\binom{2r - |I|}{2}} \cdot 2^{-|I|(2r-|I|)}\binom{n-|I|}{2r - |I|} = 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|}$
\item $2^{-\binom{2r - |I|}{2}} \cdot \frac{(2r - |I|)\Delta_{I}(E_{|I|})^{2r-|I|-1}}{(2r-|I|)!} = 
2^{-\binom{2r - |I|}{2}} \cdot \frac{(n-|I|)^{2r-|I|-1}\Delta_{I}}{2^{-(2r-|I|-1)|I|}(2r-|I|-1)!} = 
2^{\binom{|I|}{2}-\binom{2r}{2} + |I|}\frac{(n-|I|)^{2r-|I|-1}}{(2r-|I|-1)!}\Delta_{I}$
\end{enumerate}
Using \lref{approximationslemma}, 
\begin{equation}\label{approxequation}
\left|2^{-\binom{2r - |I|}{2}}\binom{|A_I|}{2r - |I|} - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|} - 
2^{\binom{|I|}{2}-\binom{2r}{2} + |I|}\frac{(n-|I|)^{2r-|I|-1}}{(2r-|I|-1)!}\Delta_{I}\right| \leq 10(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1}
\end{equation}
Using Corollary \ref{approximationscorollary},
\begin{equation}\label{corollaryequation}
\left|2^{-\binom{2r - |I|}{2}}\binom{|A_I|}{2r - |I|} - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|}\right| \leq 5(\ln(\frac{6}{\epsilon}))n^{2r-|I|-\frac{1}{2}}
\end{equation}
Now note that by equation \ref{deggiequation}, 
$$\pr\left[\left|deg_G(I) - 2^{-\binom{2r - |I|}{2}}\binom{|A_I|}{2r - |I|}\right| > 
(\ln(\frac{128}{\epsilon}))^2 \cdot |A_I|^{2r-|I|-1}\right] < \frac{\epsilon}{2}$$
Since $\ln(\frac{128}{\epsilon}) \leq 3\ln(\frac{6}{\epsilon})$ and $|A_I| \leq n$, we have that 
$$\pr\left[\left|deg_G(I) - 2^{-\binom{2r - |I|}{2}}\binom{|A_I|}{2r - |I|}\right| > 
10(\ln(\frac{6}{\epsilon}))^2 \cdot n^{2r-|I|-1}\right] < \frac{\epsilon}{2}$$
\end{proof}
Combining this with equation \ref{approxequation} which holds with probability at least $1 - \frac{\epsilon}{2}$ and using the union bound, we have that 
$$P\left[\left|deg_G(I) - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|} - 
2^{\binom{|I|}{2}-\binom{2r}{2} + |I|}\frac{(n-|I|)^{2r-|I|-1}}{(2r-|I|-1)!}\Delta_{I}\right| > 20(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1}\right] < \epsilon$$
Combining this with equation \ref{corollaryequation} which holds with probability at least $1 - \frac{\epsilon}{2}$ and using the union bound, we have that 
$$P\left[\left|deg_G(I) - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|}\right| > 10(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1} + 5(\ln(\frac{6}{\epsilon}))n^{2r-|I|-\frac{1}{2}}\right] < \epsilon$$
Following the same logic used in the proof of Corollary \ref{approxcorollary}, $10(\ln{(\frac{6}{\epsilon})})^2n^{2r-|I|-1} < 3(\ln(\frac{6}{\epsilon}))n^{2r-|I|-\frac{1}{2}}$ so we have that 
$$P\left[\left|deg_G(I) - 2^{\binom{|I|}{2}-\binom{2r}{2}}\binom{n-|I|}{2r - |I|}\right| > 8(\ln(\frac{6}{\epsilon}))n^{2r-|I|-\frac{1}{2}}\right] < \epsilon$$
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "stoc"
%%% End: 


==> technicalgeneral.tex <==
% !TEX root = main.tex

\section{Bounding norms of locally random matrices}\label{sec:localrand}
In this section we shall develop tools for bounding the norms of \emph{locally random} matrices (recall their informal definition from \sref{sec:outline} and more formal one in \sref{sec:normboundL}) associated with random graphs $G \lfta G(n,1/2)$, proving \clref{clm:maintechnicalL}. The idea behind our bounds is to use the \emph{trace method}. Recall the trace method: for any matrix $M$, for any positive integer $q$, $||M|| \leq \sqrt[2q]{tr(({M^T}M)^{q})}$ so we can probabilistically bound $||M||$ by bounding $\ex\sbkets{tr(({M^T}M)^{q})}$.

Going back to \clref{clm:maintechnicalL} let us first look at the special case of $a=1$ to gain some intuition. In this case, the entries of $R_1$ are (essentially) independent, and so the trace method is easy to apply. More precisely, $R_1$ is a symmetric random matrix with zeros on the diagonal and the entries in the upper diagonal taking independent uniformly random $\pm{1}$ values. It is well known that $\|R_1\| = O(\sqrt{n})$ in this case (see \cite{Vershynin06} for instance). One can also prove the bound by the trace method as follows. We have that  
$$\ex\sbkets{tr(({{R_1}^T}{R_1})^{q})} = \ex\sbkets{tr({R_1}^{2q})} = \sum_{i_1,\cdots,i_{2q}}{\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}},$$ where $i_{2q+1} = i_1$. We can then look at which products $\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}$ have expectation $0$. 

Since each individual ${R_1}({i_j},i_{j+1})$ is an independent $\pm{1}$ random variable with expectation $0$, a term in the summation $\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}} = 0$ unless every ${R_1}({i_j},i_{j+1})$ appears an even number of times in the product. Thus, the vast majority of the terms $\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}$ are $0$ and we can count the remaining terms to bound $\ex\sbkets{tr(R_1^{2q})}$.

\anote{Revised}

%One way to visualize the above argument is to first look at terms $\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}$ which have non-zero expectation. We observe that in all such terms, the number of distinct entries in $\{i_j: j =1,\ldots,2q\}$ is at most $q+1$. We can then bound the number of terms with non-zero expected value by the number of possible terms which contain at most $q+1$ distinct elements. This number can be easily bounded by $O((nq)^{q+1})$, so after picking $q$ optimally results in showing that with high probability $\|R_1\| = O(\sqrt{n}\log n)$, a near-optimal bound. 

One way to visualize the above argument is to take terms $\ex\sbkets{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}$ and build a ``constraint graph'' for each term where the vertices correspond to the entries $\{i_j,i_{j+1}\}$, $j = 1,\ldots,2q$ appearing in the term. We then add edges between the vertices if the corresponding sets overlap (as a proxy for the dependence of the entries in $R$ - this happens here only if the same entry $(i,j)$, or its symmetric image $(j,i)$ appear in the term more than once). It is easy to argue now that the constraint graph of any term with non-zero expectation has at most $q+1$ connected components. We can then bound the number of terms with nonzero expected value by the number of possible constraint graphs with at most $q+1$ connected components. This number can be bounded by $O((nq)^{q+1})$, so after picking the parameter $q$ optimally results in showing that with high probability  $\|R_1\| = O(\sqrt{n}\log n)$, a near-optimal bound.

To handle higher $a$'s we first generalize the above argument based on constraint graphs to work with general locally-random matrices. However, unlike for $a=1$, distinct entries of the matrix are now dependent, which significantly complicates the structure of the constraint graphs and the associated count of the terms which have non-zero expectation. The rest of the section is devoted to this. While we apply our arguments to the particular locally-random matrices arising in our proof, these techniques should apply more generally to other locally-random matrices.  

%In this section we generalize these ideas to bound $||R_a||$ in two steps. In \sref{constraintgraphs} we develop tools for bounding the trace of high powers of locally random matrices. In \sref{rabounds} we apply these tools to the matrices $\{R_a\}$.
%--------------------------------------------------------------------------%
\subsection{Constraint graphs}\label{constraintgraphs}
%--------------------------------------------------------------------------%
We now formally introduce constraint graphs, which are a useful way to visualize terms in our calculations. We then prove a generic result bounding traces of high powers of locally random matrices (and some other functions) based on the structure of the associated constraint graphs; the advantage being that the conditions on the constraint graphs (in the form of bounds on the number of connected components) will be easier to ascertain in our applications. While the statement of the main theorem does not involve constraint graphs, thinking in terms of constraint graphs is helpful in proving the conditions required to apply the theorem. 

Here we use $V$ rather than $I$ for subsets because we will be viewing the individual elements of each $V$ as vertices.
\begin{definition}
Given a family of sets of vertices $\{V_i\}$, we define a corresponding constraint graph $C$ where
\begin{enumerate}
\item $V(C_{\{V_i\}}) = \{(V_i,j): j \in V_i\}$.
\item $E(C_{\{V_i\}}) = \{((V_{i_1},j),(V_{i_2},j)): j \in V_{i_1}, j \in V_{i_2}, V_{i_1} \neq V_{i_2}\}$.
\end{enumerate}
\end{definition}
\begin{theorem}\label{thm:productgraphtonorm}
Assume that we have values $\{s_1, \cdots, s_t\}$, a constant $B > 0$, and a function $p(G,2q)$ such that for every positive $q$, $p(G,2q) \geq 0$ and $p(G,2q)$ can be written in the form $p(G,2q) = \sum_{\{V_{ij}\}}{f(G,\{V_{ij}\})}$ where the following are true
\begin{enumerate}
\item $\{V_{ij}\}$ ranges over $i \in [1,q]$, $j \in [1,t]$, and subsets of vertices $V_{ij} \subseteq V(G)$
\item For all $i$ and $j$, $|V_{ij}| = s_j$
\item Taking $x = \sum_{j}{s_j}$ so that $qx$ is the total number of vertices in each constraint graph, for every term $f(G,\{V_{ij}\})$ with nonzero expected value, $|\cup_{i,j} V_{ij}| \leq qx-qy+z$ for some integers $y$ and $z$ where $1 \leq y \leq x$ and $z \geq 0$. Equivalently, the corresponding constraint graph has at most $qx-qy+z$ connected components. 
\item $\forall i,j, \ex[f(G,\{V_{ij}\})] \leq B^{2q}$
\end{enumerate}
then if $n \geq 10$, for all $\epsilon \in (0,1)$, 
$$\pr\left[|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}} \cdot \left(ex\Big(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\Big)\right)^y \cdot n^{\frac{x-y}{2}}\right] < \epsilon$$
\end{theorem}
\begin{remark}
We will use this theorem with two types of functions $p$. When $p(G,2q) = tr(({M^T}M)^q)$ for some matrix $M$ depending on $G$, 
$||M|| \leq \sqrt[2q]{p(G,2q)}$ for all $q > 0$ so this theorem gives us a probabilistic bound on $||M||$. When $p(G,2q) = h(G)^{2q}$ for some function $h$, then $h(G) = \sqrt[2q]{p(G,2q)}$ for all $q \in \mathbb{Z}^{+}$ so this theorem gives us a probabilistic bound on $h(G)$.
\end{remark}
\begin{example}
In the case when $p(G,2q) = tr(R_1^{2q})$, $p(G,2q) = \sum_{i_1,\cdots,i_{2q}}{\prod_{j=1}^{2q}{{R_1}({i_j},i_{j+1})}}$. Each term here has expected value at most $1$ and its corresponding constraint graph has 2q vertices. It can be shown 
(see \lref{lem:connectedcomponentbound}) that for any term with nonzero expected value, the number of distinct elements is at most $q+1$. Applying \tref{thm:productgraphtonorm} with $t = 2$, $\{s_1,s_2\} = \{1,1\}$, $V_{kl} = \{i_{2k+l-2}\}$, $x = 2$, $y = z = 1$, and $B = 1$ we have that if $n \geq 10$, for all $\epsilon \in (0,1)$, 
$$\pr\left[||R_1|| > 2e\sqrt{n} (\ln{n/\epsilon} + 2) \right] < \epsilon$$
This bound is weaker (by the logarithmic factor) than the bounds in e.g. \cite{Vershynin06}, but is sufficient for our purposes.
\end{example}

\begin{proof}[Proof of \tref{thm:productgraphtonorm}]
We prove this result by obtaining an upper bound on the number of terms in $p(G,2q) = \sum_{\{V_{ij}\}}{f(G,\{V_{ij}\})}$ with nonzero expected value. This gives us a probabilistic upper bound for $p(G,2q)$, implying the upper bound on $\min_q{\{\sqrt[2q]{p(G,2q)}\}}$.
\begin{definition}
Define $N(n,\{s_1,\cdots,s_t\},q,m)$ to be the number of ways to choose subsets $\{V_{ij}: i \in [1,q], j \in [1,t]\}$ of $[n]$ such that $|\cup_{ij}{V_{ij}}| \leq m$ and for all $i,j$, $|V_{ij}| = s_j$.
\end{definition}
\begin{lemma}\label{tboundlemma}
Letting $x = \sum_{j}{s_j}$, if $m \leq qx$ then 
$$N(n,\{s_1,\cdots,s_t\},q,m) \leq \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}{\binom{qx}{qx-m}}{n^{m}}{{m}^{qx-m}}$$
\end{lemma}
\begin{proof}
We can choose each ordered $qx$-tuple $(v_1, \cdots, v_{qx})$ of elements in $[n]$ which contains at most $m$ distinct elements as follows. 
There must be at least $k-m$ elements which are duplicates of other elements, so we can first choose a set $I$ of $k-m$ indices such that for all $i \in I$, $v_i = v_j$ for some $j \notin I$. There are $\binom{qx}{qx-m}$ choices for $I$. We then choose the elements $\{v_j: j \notin I\}$. There are no restrictions on these elements so there are $n^{m}$ choices for these elements. Finally, we choose the elements $\{v_i: i \in I\}$. To determine each $v_i$ it is sufficient to specify the $j \notin I$ such that 
$v_i = v_j$. For each $i$ there are $m$ choices for the corresponding $j$, so the number of choices for these elements 
is at most $m^{qx-m}$. Putting everything together, the total number of choices is at most $\binom{qx}{qx-m}{n^{m}}{{m}^{qx-m}}$. Now note that since we are choosing subsets $\{V_{ij}: i \in [1,2q], j \in [1,t]\}$ of $[n]$ rather than one big ordered tuple, the order within each subset does not matter. Thus, there are $\left(\prod_{j=1}^{t}{{s_j}!}\right)^{2q}$ different ordered tuples which give the same subsets of elements, so the total number of possibilities for the subsets $\{V_{ij}\}$ is at most $\left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}{\binom{qx}{qx-m}}{n^{m}}{{m}^{qx-m}}$, as needed
\end{proof}
Now $\ex[p(G,2q)] = \sum_{\{V_{ij}\}}{\ex[f(G,\{V_{ij}\})]}$. For every nonzero term $\ex[f(G,\{V_{ij}\})]$, we have that $|\cup_{i,j} V_{ij}| \leq qx-qy+z$. If $q > \frac{z}{y}$ then applying \lref{tboundlemma} with $m = qx - qy + z$, the number of non-zero terms $\ex[f(G,\{V_{ij}\})]$ is at most 
\begin{align*}
\left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}\binom{qx}{qx-m}{n^{m}}{{m}^{qx-m}} &\leq 
\left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}{(qxm)}^{qx-m}{n^m} \\
&= \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}(qxm)^{yq}(qxm)^{-z}n^{(x-y)q}n^{z} \\
&= \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}(\frac{n}{qxm})^{z}\left((qxm)^{y}n^{x-y}\right)^{q} \\
&\leq \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}n^{z}\left((q^2x^2)^{y}n^{x-y}\right)^{q}.
\end{align*}
Moreover, by our assumptions, each of these nonzero terms $E[f(G,\{V_{ij}\})]$ has value at most $B^{2q}$, so $$E[p(G,2q)] \leq \left(\prod_{j=1}^{t}{\frac{1}{{s_j}!}}\right)^{q}n^{z}\left((q^2x^2)^{y}n^{x-y}\right)^{q}B^{2q}.$$
Thus, for all $q > \frac{z}{y}$, 
$$E[p(G,2q)] \leq n^{z}\left(B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}}(qx)^{y}n^{\frac{x-y}{2}}\right)^{2q}.$$
Using Markov's inequality, 
$$\epsilon > P\left(|p(G,2q)| > \frac{1}{\epsilon}E[p(G,2q)]\right) \geq P\left(|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > 
\sqrt[2q]{\frac{1}{\epsilon}E[p(G,2q)]}\right).$$
Combining these two equations gives
$$P\left(|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > \frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}} \bkets{B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}}x^{y}n^{\frac{x-y}{2}}}\right) < \epsilon.$$
We will try to minimize $\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}}$ with respect to $q$. 
Setting the derivative to $0$ gives 
$$\left(\frac{y}{q} - \frac{z\ln{n} - \ln{\epsilon}}{2q^2}\right)
\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}} = 0.$$
This occurs when $q = \frac{z\ln{n} - \ln{\epsilon}}{2y}$. We need $q$ to be an integer so we set $q$ to be the smallest 
integer which is at least $\frac{z\ln{n} - \ln{\epsilon}}{2y}$. As long as $n \geq 10$ this guarantees that $q > \frac{z}{y}$. 
Now $q < \frac{z\ln{n} - \ln{\epsilon}}{2y} + 1$ and 
$$\left(\frac{n^z}{\epsilon}\right)^{\frac{1}{2q}} \leq 
\left(e^{z\ln{n} - \ln{\epsilon}}\right)^{\frac{y}{z\ln{n} - \ln{\epsilon}}} = e^y.$$
Thus, for this $q$, 
$$\frac{q^{y}n^{\frac{z}{2q}}}{{\epsilon}^{\frac{1}{2q}}} \leq e^y\left(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\right)^y.$$
Putting everything together, 
$$P\left(|\min_{q \in \mathbb{Z}^{+}}{\{\sqrt[2q]{p(G,2q)}\}}| > e^y\left(\frac{z\ln{n} - \ln{\epsilon}}{2y} + 1\right)^y
(B\sqrt{\prod_{j=1}^{t}{\frac{1}{{s_j}!}}}x^{y}n^{\frac{x-y}{2}})\right) < \epsilon$$
and rearranging gives the desired result.
\end{proof}
%--------------------------------------------------------------------------%
\subsection{Bounds on $||R_a||$}\label{rabounds}
%--------------------------------------------------------------------------%
In this subsection, we prove \clref{clm:maintechnicalL} using \tref{thm:productgraphtonorm}. For convenience, we restate \clref{clm:maintechnicalL} here with more precise constants.
\begin{theorem}\label{th:rabounds}
If $n \geq 100$, for all $\epsilon \in (0,1)$, 
$\pr\left[||R_a|| > 2^{a^2+2a+2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon$.
\end{theorem}

We prove the theorem by applying \tref{thm:productgraphtonorm}. The core of the argument will be to bound $|\cup_{j=1}^{2q} V_{i_j}|$ for any term $\prod_{j=1}^{2q} R_a(V_{i_j}, V_{i_{j+1}})$ with non-zero expectation which appear in the expansion of $tr((R_a^T R_a)^q)$. We will do so by arguing that the constraint graph associated with the term has at most $2aq-q+1$ connected components. We will prove this bound by inductively decomposing $R_a$ as follows. 
%To make the proof cleaner, we further decompose $R_a$ as follows.
\begin{definition}
Given a partition $(A,B)$ of $[1,n]$, define $R_{a,A,B}(V_1,V_2) = R_{a}(V_1,V_2)$ if $V_1 \subseteq A$ and $V_2 \subseteq B$ and $0$ otherwise.
\end{definition}
\begin{proposition}
$\sum_{A,B}{R_{a,A,B}} = 2^{n-2a}R_a$
\end{proposition}
\begin{proof}
$R_{a,A,B}(V_1,V_2) = R_a(V_1,V_2) = 0$ whenever $V_1$ and $V_2$ are not disjoint. For all disjoint $V_1$ and $V_2$, $R_{a,A,B}(V_1,V_2) = R_a(V_1,V_2)$ for $2^{n-2a}$ choices of $A$ and $B$ and is $0$ for the rest.
\end{proof}
\begin{corollary}\label{cor:parttowhole}
$||R_a|| \leq 2^{2a}\max_{A,B}{\{||R_{a,A,B}||\}}$
\end{corollary}
\begin{proof}
Since $R_a = 2^{2a-n}\sum_{A,B}{R_{a,A,B}}$, $||R_a|| \leq 2^{2a-n}\sum_{A,B}{||R_{a,A,B}||} \leq 2^{2a}\max_{A,B}{\{||R_{a,A,B}||\}}$
\end{proof}
Now given $A$ and $B$, take 
\begin{align*}
p(G,2q) = tr((R^T_{a,A,B}R_{a,A,B})^q) &= \sum_{\{V_{ij}: i \in [1,q], j \in [1,2]\}}{\prod_{i=1}^{q}{R^T_{a,A,B}(V_{i1},V_{i2})R_{a,A,B}(V_{i2},V_{(i+1)1})}} \\
&= \sum_{{\{V_{ij}: i \in [1,q], j \in [1,2]\}: \atop \forall i, V_{i1} \subseteq B} \atop {\forall i, V_{i2} \subseteq A}}
{\prod_{i=1}^{q}{R_{a}(V_{i1},V_{i2})R_{a}(V_{i2},V_{(i+1)1})}}
\end{align*} 
where we take $V_{(q+1)1} = V_{11}$. 

To simplify this expression, rename the sets of vertices as follows.
\begin{definition} \ 
\begin{enumerate}
\item If $i \in [1,2q]$ and $i$ is odd then take $W_i = V_{(\frac{i+1}{2})1}$
\item If $i \in [1,2q]$ and $i$ is even then take $W_i = V_{(\frac{i}{2})2}$
\end{enumerate}
\end{definition}
We now have that 
\begin{equation}\label{eq:termab}
p(G,2q) = \sum_{{{\{W_i}: i \in [1,2q]\}: \atop \forall \text{ odd } i, W_{i} \subseteq B} \atop {\forall \text { even } i, W_{i} \subseteq A}}{\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}},
\end{equation}
where we take $W_{2q + 1} = W_1$. Now let's consider which of these terms have expectation $0$. Each $R_{a}(W_{i},W_{i+1})$ is a random variable with expectation $0$, so if any $R_{a}(W_{i},W_{i+1})$ is independent from everything else, the product will have expectation $0$. Each $R_{a}(W_{i},W_{i+1})$ is independent from everything else precisely when none of the edges between $W_{i}$ and $W_{i+1}$ appear anywhere else. Thus, we only need to count the terms such that for all $i$ there is a $j \neq i$ such that some edge between $W_{i}$ and $W_{i+1}$ is also an edge between $W_{j}$ and $W_{j+1}$.

We express this condition in terms of the constraint graphs as follows. We first define a related graph $H$ which is easier to work with and analyze.
\begin{definition}
Given a constraint graph $C$, let $H$ a graph with two types of edges, product edges and constraint edges, such that 
\begin{enumerate}
\item $V(H) = \{W_i: i \in [1,2q]\}$
\item $E_{product}(H) = \{(W_i,W_{i+1}): i \in [1,2q]\}$
\item $E_{constraint}(H) = \{(W_i,W_j): i \neq j, W_i \cap W_j \neq \emptyset\}$
\end{enumerate}
\end{definition}
We now define the concept of an independence breaking cycle on $H$ so that for each $i$, 
there is a $j \neq i$ such that some edge is both between $W_i$ and $W_{i+1}$ and between $W_j$ and $W_{j+1}$ if and only if the product edge $(W_{i},W_{i+1})$ is part of an independence-breaking cycle. This implies each product $\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}$ has zero expected value unless all of the product edges in the corresponding $H$ are part of independence-breaking cycles. This places restrictions on $H$ (see \lref{lem:connectedcomponentbound}) which in turn places restrictions on the constraint graph $C$, allowing us to use \tref{thm:productgraphtonorm}. We make these ideas precise below.
\begin{definition}
Given $q$ and $\{W_1, \cdots, W_{2q}\}$, we define $W_{i \pm 2q} = W_{i}$ for all $i \in [1,2q]$.
\end{definition}
\begin{definition} If $q \geq 2$, 
\begin{enumerate}
\item Define an independence breaking 3-cycle in $H$ to consist of product edges $(W_i,W_{i+1})$, $(W_{i+1},W_{i+2})$ 
and a constraint edge $((W_{i},j),(W_{i+2},j))$.
\item Define an independence breaking 4-cycle to consist of product edges $e_1 = (W_{i_1},W_{i_1+1})$, 
$e_2 = (W_{i_2},W_{i_2 \pm 1})$ and constraint edges $(W_{i_1},W_{i_2})$ and $(W_{i_1 + 1},W_{i_2 \pm 1})$.
\end{enumerate}
\end{definition}
\begin{proposition}
For all $W_1, \cdots, W_{2q}$ such that $W_i \subseteq B$ whenever $i$ is odd and $W_i \subseteq A$ whenever $i$ is even, if the corresponding $H$ has a product edge $(W_i,W_{i+1})$ which is not contained in any independence-breaking cycle then $E[\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}] = 0$
\end{proposition}
\begin{proof}
If $(W_i,W_{i+1})$ is not contained in any independence-breaking cycle then no edge between $W_i$ and $W_{i+1}$ appears anywhere else so $R_{a}(W_{i},W_{i+1})$ is a random variable with expectation $0$ which is independent from everything else and thus $E[\prod_{i=1}^{2q}{R_{a}(W_{i},W_{i+1})}] = 0$.
\end{proof}
We now bound the number of connected components in $H$ with the following lemma.
\begin{lemma}\label{lem:connectedcomponentbound}
If $q \geq 2$ and $H$ is a graph such that
\begin{enumerate}
\item Every product edge of $H$ is contained in an independence-breaking cycle.
\item Every constraint edge of $H$ is of the form $(W_i,W_{i+j})$ where $j$ is even.
\end{enumerate} 
then looking only at the constraint edges, the number of connected components of $H$ is at most $q+1$.
\end{lemma}
The intuitive idea behind this lemma is that if we add the constraint edges in the right order, every new constraint edge can put two product edges into independence breaking cycles. For example, a constraint edge between $W_{i-1}$ and $W_{i+1}$ puts the product edges $(W_{i-1},W_i)$ and $(W_i,W_{i+1})$ into an independence breaking 3-cycle. If we then add a constraint edge between $W_{i-2}$ and $W_{i+2}$, this puts the product edges $(W_{i-2},W_{i-1})$ and $(W_{i+1},W_{i+2})$ into an independence breaking 4-cycle. The final constraint edge can put 4 product edges into independence breaking cycles, so the number of constraint edges needed is $q-1$.

To make this argument work, we use an inductive proof. We note that if there is no $W_i$ which is isolated in $H$, we must have at least $q$ constraint edges. On the other hand, if there a $W_i$ which is isolated, there must be a constraint edge between $W_{i-1}$ and $W_{i+1}$. As noted above, this constraint edge puts the product edges $(W_{i-1},W_i)$ and $(W_i,W_{i+1})$ into an independence breaking 3-cycle. We take this to be the first constraint edge. We then argue that we can essentially delete $W_i$ and merge $W_{i-1}$ and $W_{i+1}$ which allows us to use the inductive hypothesis. We make these ideas rigorous below.
\begin{proof}[Proof of \lref{lem:connectedcomponentbound}]
We prove \lref{lem:connectedcomponentbound} by induction on $q$. The base case $q = 2$ is trivial, as we clearly need at least one constraint edge, so the number of connected components in $H$ is at most $3$. 
Now assume that $q = k \geq 3$ and the result is true for $q = k-1$.

First note that if there is no $W_i$ which is isolated (when looking only at constraint edges), then there are at most 
$q$ connected components in $H$. Thus, we may assume that $W_i$ is isolated for some $i$. Now 
note that for the product edge $(W_{i-1},W_{i})$, since $W_i$ is isolated, there are no independence breaking 3-cycles or 4-cycles where $W_i$ is the endpoint of a constraint edge. 
Thus, we must have that $(W_{i-1},W_{i})$ is part of an independence breaking 3-cycle consisting of $(W_{i-1},W_i)$, $(W_i,W_{i+1})$, and 
a constraint edge $(W_{i-1},W_{i+1})$.

Now form a new graph $H'$ as follows. Delete $W_i$ and contract the constraint edge between $W_{i-1}$ and $W_{i+1}$. More precisely, 
\begin{enumerate}
\item Take $V(H') = V(H) \setminus \{W_{i-1},W_i,W_{i+1}\} \cup \{U\}$
\item Take $E_{product}(H') = E_{product}(H) \setminus \{(W_{j},W_{j+1}): j \in [i-2,i+1]\} \cup \{(W_{i-2},U),(U,W_{i+2})\}$
\item Take \begin{align*}
E_{constraint}(H') &= E_{constraint}(H) \setminus \{(W_{i-1},W_{j}): (W_{i-1},W_{j}) \in E_{constraint}(H)\} \\
&\setminus \{(W_{i+1},W_{j}): (W_{i+1},W_{j}) \in E_{constraint}(H)\} \\
&\cup \{(U,W_{j}): (W_{i-1},W_{j}) \in E_{constraint}(H) \text{ or } (W_{i+1},W_{j}) \in E_{constraint}(H)\}
\end{align*}
\end{enumerate}
After doing this, rename $U$ as $W_{i-1}$ and rename each $W_{j}$ where $j > i+1$ as $W_{j-2}$. In going from $H$ to $H'$, we have effectively reduced both $q$ and the number of connected components by $1$. To complete the proof, we need to check that $H'$ satisfies the inductive hypotheses. Based on the reduction from $H$ to $H'$, we still have that every constraint edge is of the form $(W_i,W_{i+j})$ where $j$ is even. We check that every product edge is still part of an independence-breaking cycle case by case. 
\begin{enumerate}
\item Every independence-breaking cycle which did not contain the constraint edge $(W_{i-1},W_{i+1})$ in $H$ is preserved in $H'$ except that the vertices may have been renamed. The reason for this is that such an independence breaking cycle in $H$ cannot contain $W_i$ and can contain at most one of $\{W_{i-1},W_{i+1}\}$.
\item The independence-breaking 3-cycle in $H$ consisting of the product edges $(W_{i-1},W_{i})$, $(W_{i},W_{i+1})$ and the constraint edge $(W_{i-1},W_{i+1})$ is removed, but so are the product edges $(W_{i-1},W_{i})$ and $(W_{i},W_{i+1})$, so this is fine.
\item If we have an independence breaking 4-cycle in $H$ consisting of the product edges $(W_{i-2},W_{i-1})$, $(W_{i+1},W_{i+2})$ and the constraint edges $(W_{i-1},W_{i+1})$, $(W_{i-2},W_{i+2})$, this becomes an independence-breaking 3-cycle in $H'$ with product edges $(W_{i-2},W_{i-1})$, $(W_{i-1},W_{i})$ and a constraint edge $(W_{i-2},W_{i})$ (note that $W_{i-1}$ and $W_{i+1}$ are merged into $W_{i-1}$ in $H'$ and $W_{i+2}$ is renamed as $W_i$ in $H'$).
\end{enumerate}
$H'$ satisfies the inductive hypotheses, so looking only at the constraint edges, $H'$ has at most $(q-1)+1 = q$ connected components. $H$ has one more connected component than $H'$ (the vertex $W_i$ in $H$), so $H$ has at most $q+1$ connected components, as needed.
\end{proof}
\begin{remark}
The fact that $W_i \subseteq B$ whenever $i$ is odd and $W_i \subseteq A$ is even saved us from considering the possibility that we had an independence breaking 4-cycles consisting of product edges $(W_{i+1},W_{i+2})$, $(W_{i-2},W_{i-1})$ and constraint edges $(W_{i-1},W_{i+2})$, $(W_{i-2},W_{i+1})$. Such an independence-breaking 4-cycle would be contracted into a 4-cycle with only three vertices. We could have modified the definition of independence-breaking 4-cylces to include this possibility, but it is cleaner and easier to think about when we avoid this case and other weird cases entirely. 
\end{remark}
We now use this bound on the number of connected components of $H$ to prove a corresponding bound on the number of connected components of $C$.
\begin{proposition}
For all constraint graphs $C$ and the corresponding graphs $H$, $|V(C)|$ minus the number of connected components of $C$ is at least as large as $|V(H)|$ minus the number of connected components of $H$.
\end{proposition}
\begin{proof}
Consider the process of starting with $V(H)$ and then adding edges of $H$ one at a time where each new edge reduces the number of connected components until this is no longer possible. The number of edges we add is $|V(H)|$ minus the number of connected components of $H$. Now note that if we start with $V(C)$ and add the corresponding edges in $C$, this already reduces the number of connected components by the number of edges we added and the result follows.
\end{proof}
\begin{corollary}
For all terms in \eref{eq:termab} with nonzero expectation, the corresponding constraint graph $C$ has at most $2aq - q + 1$ connected components 
\end{corollary}
We can now prove \tref{th:rabounds}
\begin{proof}[Proof of \tref{th:rabounds}]
We can now apply \tref{thm:productgraphtonorm} with $t=2$, $s_1 = s_2 = a$, $x = 2a$, $y = 1$, and $z = 1$. Every entry of $R_{a,A,B}$ has magnitude at most $2^{a^2}$ so we can take $B = 2^{a^2}$. By \tref{thm:productgraphtonorm}, if $n \geq 10$, for all $A$ and $B$, for every $\epsilon \in (0,1)$, 
$$\pr\left[||R_{a,A,B}|| > \frac{2^{a^2}}{a!}\left(2ea\Big(\frac{\ln{n} - \ln{\epsilon}}{2} + 1\Big)\right)
n^{\frac{2a-1}{2}}\right] = 
\pr\left[||R_{a,A,B}|| > \frac{2^{a^2}ea}{a!}(\ln{n} - \ln{\epsilon} + 2)
n^{a - \frac{1}{2}}\right] < \epsilon$$
Since $4\ln{n} \geq e(\ln{n} + 2)$ for all $n \geq 100$ and $a! \geq a$, we have that for all $n \geq 100$, for all $A$ and $B$ and all $\epsilon \in (0,1)$, 
$$\pr\left[||R_{a,A,B}|| > 2^{a^2+2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon$$
Now by \cref{cor:parttowhole}, $||R_a|| \leq 2^{2a}\max_{A,B}{\{||R_{a,A,B}||\}}$ so $$\pr\left[||R_{a}|| > 2^{a^2 + 2a + 2}\ln{(\frac{n}{\epsilon})}n^{a - \frac{1}{2}}\right] < \epsilon$$
\end{proof}

%%% Local Variables:   
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

